SaVeR: Optimal Data Collection Strategy for Safe Policy Evaluation in Tabular MDP

In this paper, we study safe data collection for the purpose of policy evaluation in tabular Markov decision processes (MDPs). In policy evaluation, we are given a \textit{target} policy and asked to estimate the expected cumulative reward it will obtain. Policy evaluation requires data and we are interested in the question of what \textit{behavior} policy should collect the data for the most accurate evaluation of the target policy. While prior work has considered behavior policy selection, in this paper, we additionally consider a safety constraint on the behavior policy. Namely, we assume there exists a known default policy that incurs a particular expected cost when run and we enforce that the cumulative cost of all behavior policies ran is better than a constant factor of the cost that would be incurred had we always run the default policy. We first show that there exists a class of intractable MDPs where no safe oracle algorithm with knowledge about problem parameters can efficiently collect data and satisfy the safety constraints. We then define the tractability condition for an MDP such that a safe oracle algorithm can efficiently collect data and using that we prove the first lower bound for this setting. We then introduce an algorithm SaVeR for this problem that approximates the safe oracle algorithm and bound the finite-sample mean squared error of the algorithm while ensuring it satisfies the safety constraint. Finally, we show in simulations that SaVeR produces low MSE policy evaluation while satisfying the safety constraint.

==> mdp.tex <==
In this section, we begin by deriving a data collection strategy assuming the variances of the reward and cost distributions are known and then analyze the finite-sample MSE of this algorithm. We denote this as an oracle strategy.



% Tree MDPs are an extension of the multi-armed bandit model that captures the fact that the optimal choice of action in a given state must consider the future states that could arise from taking that action. 
% % \par
% We first define a discrete tree MDP as:
% \begin{definition}\textbf{(Tree MDP)}
% \label{def:tree-mdp}
% An MDP is a discrete tree MDP $\T\subset \M$ in which:
% \par
% \textbf{(1)} There are $L$ levels indexed by $\ell$ where $\ell = 1,2,\ldots,L$. 
% % \par
% \textbf{(2)} Every state is represented as $s^\ell_i$ where $\ell$ is the level of the state $s$ indexed by $i$. 
% % \par
% \textbf{(3)} The transition probabilities are such that one can only transition from a state in level $\ell$ to one in level $\ell + 1$ and each non-initial state can only be reached through one other state and only one action in that state. Formally, $\forall s'$, $P(s' | s,a) \neq 0$ for only one state-action pair $s,a$ and if $s'$ is in level $\ell + 1$ then $s$ is in level $\ell$. Finally, $P(s^{L+1}_j|s^L_i, a) = 0, \forall a$.
% % \par
% \textbf{(4)} For simplicity, we assume that there is a single starting state $s^1_1$ (called the root). It is easy to extend our results to multiple starting states with a starting state distribution, $d_0$, by assuming that there is only one action available in the root that leads to each possible start state, $s$, with probability $d_0(s)$. The leaf states are denoted as $s^L_i$. %Note that each episode has a horizon of $L$ from root $s^1_1$ to an arbitrary leaf state $s^L_i$.
% % \par
% \textbf{(5)} The interaction stops after $L$ steps in state $s^L_i$ after taking an action $a$.
% % and observing the reward $R_L(s^L_i,a)$.
% \end{definition}
% Note that, because we assume a single initial state, $s_1^1$, we have that estimating $V_\pi$ is equivalent to estimating $V_\pi(s_1^1)$.
% A similar Tree MDP model has been previously used in the theoretical analysis by \citet{jiang2016doubly}; our model is slightly more general as we consider per-step stochastic rewards whereas \citet{jiang2016doubly} only consider deterministic rewards at the end of trajectories. We assume $\pi_0$ is a deterministic mapping from states to actions and we assume w.l.o.g. that in any state $\pi_0$ takes action $0$.
% % Finally, note that when $\pi_0$ is run from the starting state $s^1_1$ it visits each state $s^\ell_j$ for $\ell\in[L]$ and samples the baseline action $\{0\}$ and returns the final estimate $V^c_{\pi_0}(s^1_1)$ to the learner. 
% Finally the learner observes $V^c_{\pi_0}(s^1_1)$. 
% For our analysis, we assume that model $P(s'|s,a)$ is known and $\gamma=1$. 

 








Denote $\bb^k$ as the policy played at episode $k$.
%
%
Now we describe the oracle-safe version of \rev for the Tree-MDP as follows: For each episode $k=1,2,\ldots,K$
\begin{align}
% \text{For each episode $k=1,2,\ldots,K$}
\quad \text{Play } \bb^k = \begin{cases} \pi_e & \text{ if }             \wZ^k \geq 0, k \leq \sqrt{K}\\
            %%%%%%%%%%%
            \pi_{\bb^{*,k}} & \text{ if } \wZ^k \geq 0, k > \sqrt{K}\\
             %%%%%%%%%%%%
            \pi_0 &\text{ if } \wZ^k < 0 \label{eq:mdp-saver-oracle-sample}
\end{cases} 
\end{align}
% &\quad\text{For each time $\ell=1,2,\ldots,L$}\nonumber\\
% %%%%%%%%%%%%%%
%     &\quad\quad\text{Play } A^k_\ell =\begin{cases}
%         \argmax_a\frac{\bb^*(a|s^\ell_j)}{T^k_\ell(s^\ell_j,a)} &\text{ if } \wZ^k \geq 0, k > \sqrt{K}\\
%         %%%%%%%%%%%%
%         \sim \pi_e & \text{ if } \wZ^k \geq 0, k \leq \sqrt{K}\\
%         %%%%%%%%%%%%
%         \pi_0 &\text{ if } \wZ^k < 0 
%     \end{cases}
% \end{align}
where $\pi_{\bb^{*,k}}$ for the episode $k$ is defined as follows: For each time $\ell=1,2,\ldots,L$ sample action $A^k_\ell = \argmax_a\frac{\bb^*(a|s^\ell_j)}{T^k_\ell(s^\ell_j,a)}$, where $\bb^*(a|s^\ell_j)$ is defined in \eqref{eq:mdp-b-def}. We define $\wZ^k \coloneqq \sum_{j=1}^{k}\underline{Y}^{c}_{\bb^j}(s^1_1)  - (1-\alpha)kV^{c}_{\pi_0}(s^1_1)$ as the safety budget as oracle does not know the cost means of the actions  and must use a lower bound in their place. 
Here, $A^k_{\ell}$ is the action sampled at episode $k$ and time $\ell$. The $\underline{Y}^{c}_{\bb^j}(s^1_1) = Y^{c}_{\bb^j}(s^1_1) - C_{\bb^j}(s^1_1)$ is the lower confidence bound to the empirical value of the policy $\bb^j$. Define $C_{\bb^j}(s^1_1)\coloneqq \sum_{(s,a)\in\H^j}(2\eta + 4\eta^2) \sqrt{\nicefrac{\log (SA n(n+1) / \delta)}{2 T^j_L(s,a)}}$ \citep{agarwal2019reinforcement}.
%
Observe that $\wZ^k$ is lower confidence bound to the true safety budget $\sum_{j=1}^k V_{\bb^{j}}^c(s_1) \geq (1-\alpha)k V^c_{\pi_0}(s_1)$. 
%
Hence, when $\wZ^k \geq 0$ the oracle follows the \rev oracle proportion $\bb^*$ when $k > \sqrt{K}$ or plays the exploration policy $\pi_e$ to build a good cost estimate of each $\mu^c(s,a)$. When the safety budget $\wZ^k < 0$ it falls back to the baseline policy and samples it to make the $\wZ^k$ positive again. We define the $M =\sum_{\ell=1}^L\sum_{s^\ell_j}M(s^\ell_j)$, and $H_* =\sum_{\ell=1}^L\sum_{s^\ell_j}H_*(s^\ell_j)$ are the problem complexity parameter summed over all stated $s\!\in\![S]$.
% %
% Also, observe that the action selection rule ensures that the ratio $\bb^*(a)/T_{t}(a) \approx 1$.
% % 
% It is a deterministic action selection rule and thus avoids variance due to simply sampling from the optimal proportions $\bb^*(a)$ and ensuring safety constraint.
%
Define the predicted oracle constraint violation as $\C_n^\star(\pi) \coloneqq \sum_{k=1}^K\indic{\wZ^k < 0}$ when taking actions according to \eqref{eq:mdp-saver-oracle-sample}. Similarly define predicted agnostic constraint violation $\C_n(\pi) \coloneqq \sum_{k=1}^K\indic{\wZ^k < 0}$ when taking actions according to \eqref{eq:mdp-saver-sample}.
%
We state the oracle MSE now.


\begin{customtheorem}{3}(\textbf{informal})
\label{thm:mdp-oracle-loss}
The MSE of the oracle in $\T$ for $\frac{n}{\log(SAn(n+1)/\delta)} \geq 32(LSA^2)^2 + \frac{SA}{\Delta^{c,(2)}_{\min}} + \frac{1}{4 H_*^2}$ is bounded by
$\L^*_n(\pi) \leq O\big(\frac{M^2(s^1_1)}{n} + \frac{M^2(s^1_1)}{n}(M LSA^2 + H_*)^2 \big) $
    % \begin{align*}
    %     &\L^*_n(\pi) \leq O\bigg(\underbrace{\frac{M^2}{n}}_{\substack{\textbf{Safe Loss,}\\\wZ^k \geq 0}} + \underbrace{\dfrac{M^2(s^1_1)}{n}\left(M LSA^2 + H_*\right)^2}_{\substack{\textbf{Unsafe Loss,}\wZ^k < 0}} \bigg) 
    % \end{align*}
    with probability $(1-\delta)$. The total predicted constraint violations are bounded by
    % \begin{align*}
        $\C^*_n(\pi) \leq \frac{H_*}{2} \frac{n}{M_{\min}} + 16  LSA^2 $
    % \end{align*}
    with probability $(1-\delta)$, where $M_{\min} \coloneqq \min_s M(s)$.
\end{customtheorem}

From \Cref{thm:mdp-oracle-loss} observe  that the first quantity is denoted as the safe MSE when the safety budget $\wZ^k \geq 0$ and scales as $M(s^1_1)^2/n$. The second quantity is denoted as the unsafe MSE which is accumulated due to constraint violation ($\wZ^k < 0$) and sampling of the safe action $0$. Comparing the result of the \Cref{thm:mdp-oracle-loss} with \citet{mukherjee2022revar} we have the additional quantity of
    $\frac{(M LSA^2 + H_*)^2}{n}$
where $H_*$ is the problem-dependent quantity summed over all states. 
%
Observe that if all actions are safe then we have that $\L^*_n(\pi) = \frac{M^2(s^1_1)}{n}$ which recovers the oracle MSE in \citet{mukherjee2022revar}.
%
Compared to the bandit result, the tree oracle MSE suffers an additional $(LSA^2)^2$ factor. This is a natural artifact of union bounding in the tabular RL setting \citep{agarwal2019reinforcement}. We leave it to future work to reduce this factor.

% \begin{proof}\textbf{(Overview)}
\textbf{Proof (Overview):} 
     First, note that in the tree MDP $\T$ we have a closed form expression of $\bb^*(s^\ell_j|a)$. 
     % So we use a similar proof technique as \Cref{thm:bandit-oracle-loss} but consider allocations across episodes $K$, horizon $L$, and states $S$. 
     We divide the total budget $n = n_f + n_u$ where $n_f$ are the samples allocated when safety budget $\wZ^k \geq 0$. The $n_f$ samples are also used by the exploration policy $\pi_e$ to ensure a good estimate of the cost means as stated in the event $\xi_{c,K}$ \eqref{eq:mdp-good-cost-event}. This is ensured by $\pi_e$ and noting that $n > SA\log(1/\delta)/\Delta^{c,(2)}_{\min}$. The remaining samples from $n_f$ are allocated for reducing the MSE by sampling according to $\argmax_a(\bb^*(a|s)/T^k_\ell(s,a))$. We again prove an upper and lower bound to $T_{n}(s,a)$ in \eqref{eq:mdp-oracle-6-1} and \eqref{eq:mdp-oracle-6-2} in step $5$. Finally using \Cref{lemma:wald-variance} we can bound the MSE for the duration $n_f$ for all actions $a\in\A\setminus\{0\}$ for each state $s^\ell_j$ in step $6$. Now for an upper bound to constraint violations, we use the gap $\Delta^{c,\alpha}(s,a)\coloneqq(1-\alpha) \mu^c_0(s,a)-\mu^c(s,a)$ to bound how much each $a\in\A\setminus\{0\}$ in $s^\ell_j$ is underpulled and their pulls replaced by action $\{0\}$ weighted by $\pi(a|s^\ell_j)\sigma(s^\ell_j,a)$. This is captured by $H_*(s)$. Summing over all $s$, and horizon $L$ gives the upper bound to the violations as shown in step $7$. Finally, we also show a lower bound to constraint violations to bound the MSE for the duration when actions $a\in\A\setminus\{0\}$ are underpulled. This is shown in steps $8$ and $9$ where we equate the safety budget to $0$ to obtain a lower bound to $T_n(s^\ell_j, 0)$ for each state $s^\ell_j$. Combining everything in step $10$ gives the result. The proof is in \Cref{app:mdp-oracle-loss}.  \hfill$\blacksquare$
% \end{proof}



% \vspace*{-1.1em}
\subsection{Agnostic Tree Algorithm}
% \vspace*{-0.4em}
In this section, we introduce the more realistic tree algorithm that does not know the mean and variances of the actions but samples according to the optimal oracle sampling rule in \eqref{eq:mdp-saver-oracle-sample} using plug-in estimates. We then analyze this algorithm and establish its regret bound against the MSE of the oracle derived in \Cref{thm:mdp-oracle-loss}. 
%
We introduce a few notations before presenting the algorithm. Define the upper confidence bound on the empirical reward variance as $\overline{\wsigma}^{k}_\ell(s,a) \coloneqq \wsigma^{k}_\ell(s,a) + C^k_\ell(s,a)$, where $C^k_\ell(s,a)$ is defined in \eqref{eq:confidence-interval}. 
%
%
We define the empirical sampling proportion for an arbitrary state-action $(s^\ell_i,a)$ as $\wb^k_\ell(a|s^{\ell}_i)$. The $\wb^k_\ell(a|s^{\ell}_i)$ is similar to $\bb^*(a|s^\ell_i)$ defined in \eqref{eq:mdp-b-def}, but we use plug-in estimate $\overline{\wsigma}^{k}_\ell(s,a)$ instead of $\sigma^{k}_\ell(s,a)$. 
%
% We define the empirical sampling proportion for an arbitrary state $s^\ell_i$:
% \begin{align}
%     \wb^k_\ell(a|s^{\ell}_i) \!&\propto
%     \!\! (\! \pi^2(a|s_i^{\ell})\! \big[\overline{\wsigma}^{k,(2)}_\ell(s,a)\!  +\! \!\!  \sum\limits_{s^{\ell+1}_j}\!\!P(s^{\ell + 1}_j|s_i^{\ell}, a) \wM^2(s^{\ell+1}_j)\! \big])^{1/2}, \label{eq:mdp-wb-def}
% \end{align}
% where, $\wM(s^{\ell}_j)$ is the normalization factor defined as follows:
% \begin{align}
%     \wM(s^{\ell}_{i}) \!\!=\!\! 
%     \sum\limits_a\!\! (\!\!\pi^2(a|s^{\ell}_{i})\!\big(\!\!\overline{\wsigma}^{k,(2)}_\ell(s,a) \!+\! \gamma^2\!\sum\limits_{s^{\ell+1}_j}\!\!P(s^{\ell+1}_j\!|\!s^{\ell}_i, a) \wM^2(s^{\ell+1}_j)\!\!\big))^{1/2}%\\
%     \label{eq:wM-def}
% \end{align}
%
%
%
Finally, we define the sampling rule at episode $k$ 
\begin{align}
\quad \text{Play } \bb^k = \begin{cases} \pi_e & \text{ if }             \wZ^k \geq 0, k \leq \sqrt{K}\\
            %%%%%%%%%%%
            \pi_{\wb^k} & \text{ if } \wZ^k \geq 0, k > \sqrt{K}\\
             %%%%%%%%%%%%
            \pi_0 &\text{ if } \wZ^k < 0 \label{eq:mdp-saver-sample}
\end{cases} 
\end{align}
where $\pi_{\wb^k}$ for the episode $k$ is defined as follows: For each time $\ell=1,2,\ldots,L$ sample action $A^k_\ell = \argmax_a\tfrac{\wb^k(a|s^\ell_j)}{T^k_\ell(s^\ell_j,a)}$, where $\wb^k(a|s^\ell_j)$ is the plug-in estimate of $\bb^*(a|s^\ell_j)$ as defined in \eqref{eq:mdp-b-def}.
% time $\ell$ as follows:
% \begin{align}
% \text{Play } A^k_\ell = \argmax_a\big({\wb^k_\ell(a|s^\ell_j)}/{T^k_\ell(s^\ell_j,a)}\big) \label{eq:mdp-saver-sample}
% % &\text{For each episode $k=1,2,\ldots,K$}\nonumber\\
% % &\quad\text{For each time $\ell=1,2,\ldots,L$}\nonumber\\
% % %%%%%%%%%%%%%%
% %     &\quad\quad\text{Play } A^k_\ell =\begin{cases}
% %         \argmax_a\frac{\wb^k_\ell(a|s^\ell_j)}{T_\ell(s^\ell_j,a)} &\text{ if } \wZ^k \geq 0, k > \sqrt{K}\\
% %         %%%%%%%%%%%%
% %         \sim \pi_e & \text{ if } \wZ^k \geq 0, k \leq \sqrt{K}\\
% %         %%%%%%%%%%%%
% %         0 &\text{ if } \wZ^k < 0 \label{eq:mdp-saver-sample}
% %     \end{cases}
% \end{align}



Now we formally state the \sav\ for the tree MDP setting. 
% in \Cref{alg:bandit-track}. 
% It takes as input the risk parameter $\alpha > 0$ and target policy $\pi$ and builds the dataset $\D$. 
At every episode $k\in[K]$ it generates a sampling history $\H^k \coloneqq \{S^k_\ell, A^k_{\ell},R^k_\ell(A^k_{\ell}),C^k_\ell(A^k_{\ell})\}_{\ell=1}^L$ by selecting $A^k_\ell$ according to \eqref{eq:mdp-saver-sample} and appends it to the dataset $\D$. 
%
%
%
After observing the feedback it updates the model parameters and estimate $\wb^{k+1}_{1}(s,a)$ for each $s,a$. Finally, it returns the dataset $\D$ to evaluate $\pi$. This pseudocode is in \Cref{alg:tree-track}.
\begin{algorithm}
\caption{\textbf{Sa}fe \textbf{V}arianc\textbf{e} \textbf{R}eduction (\sav) for $\T$}
\label{alg:tree-track}
\begin{algorithmic}[1]
\State \textbf{Input:} Risk Parameter $\alpha>0$, target policy $\pi$.
\State \textbf{Output:} Dataset $\D$.
\State Initialize $\D = \emptyset$, $\wb^{}_1(a|s)$ uniform over all actions.
\For{$k=1,2,\ldots,K$}

\For{$\ell=1,2,\ldots,L$}
\State Generate $\H^k \coloneqq \{S^k_\ell, A^k_{\ell},R^k_\ell(A^k_{\ell}),C^k_\ell(A^k_{\ell}\}_{\ell=1}^L$ by selecting \indent$A^k_\ell$ according to \eqref{eq:mdp-saver-sample}.
\State $\D \leftarrow \D \cup \{(\H^k, \wb^k)\}$
\State Update model parameters and estimate $\wb^{k+1}_{1}(a|s)$ for \indent each $s,a$ 
% such that $\wb^k_{\ell+1}(a|s) \coloneqq \pi(a)\overline{\wsigma}^2_{\ell+1}(s,a)$. 
% \State Update $\wb^{}_{\ell}(a)$ following \eqref{eq:bandit-bhat} for each action $a$ .
\EndFor
\EndFor
\State \textbf{Return} Dataset $\D$ to evaluate policy $\pi$.
\end{algorithmic}
\end{algorithm}

We now present the MSE of the agnostic algorithm \sav\ in the tree MDP in the following theorem.

\begin{customtheorem}{4}\textbf{(informal)}
\label{thm:mdp-agnostic-loss}
The MSE of the \sav\ in $\T$ for $\frac{n}{\log(SAn(n+1)/\delta)} \!\!\geq\!\! 32(LSA^2)^2 + \tfrac{SA}{\Delta^{c,(2)}_{\min}} + \tfrac{1}{4 H_*^2}$ is bounded by $\L_n(\pi) \leq O\big(\tfrac{M^2(s^1_1)}{n} + \frac{M^2(s^1_1)}{n}(M LSA^2 + H_*)^2   + \tfrac{(LSA^2)^2 H_*^2 M^2\sqrt{\log (n)}}{\min_{s}\bb^{*,k,(3/2)}(s)n^{3/2}}\big)$
    % \begin{align*}
    %     &\L_n(\pi) \leq O\bigg(\underbrace{\frac{M^2(s^1_1)}{n}}_{\substack{\textbf{Safe Loss,}\\\wZ^k \geq 0}} + \underbrace{\dfrac{M^2(s^1_1)}{n}\left(M LSA^2 + H_*\right)^2}_{\substack{\textbf{Unsafe Loss,}\wZ^k < 0}} \bigg) \nonumber\\
    %     %%%%%%%%%%%%%%
    %     & \quad + O\left(\dfrac{L^2S^2A^4 H_*^2 M^2\sqrt{\log (n)}}{\min_{s}\bb^{*,k,(3/2)}(s)n^{3/2}}\right)
    % \end{align*}
    with probability $(1-\delta)$. 
    % The $M =\sum_{\ell=1}^L\sum_{s^\ell_j}M(s^\ell_j)$, and $H_* =\sum_{\ell=1}^L\sum_{s^\ell_j}H_*(s^\ell_j)$ is the problem complexity parameter. 
    The total predicted constraint violations are bounded by
    % \begin{align*}
        $\C_n(\pi) \leq O\big(\frac{H_*}{2} \frac{n}{M_{\min}} + LSA^2 +  \frac{(LSA^2)^2 H_*^2 M^2\sqrt{\log (n)}}{n^{1/2}}\big)$
    % \end{align*}
    with probability $(1-\delta)$, where $M_{\min} \coloneqq \min_s M(s)$.
\end{customtheorem}

% \begin{proof}\textbf{(Overview)}
\textbf{Proof (Overview)}
    The agnostic \sav\ does not know the reward variances. The sampling rule in \eqref{eq:mdp-saver-sample} ensures that the good variance event $\xi_{v,K}$ in \eqref{eq:mdp-good variance-event} holds such that \sav\ has good estimates of reward variances. The remaining  
    proof follows the same steps as \Cref{thm:mdp-oracle-loss} where we plug-in the upper bound to $\sigma(s,a)$ for each $s,a$. The proof is in \Cref{app:mdp-saver-loss}. $\blacksquare$
% \end{proof}

From the result of \Cref{thm:mdp-agnostic-loss} we can show that the agnostic \sav\ suffers an additional MSE factor that scales as $\tfrac{(LSA^2)^2\sqrt{\log (SA n(n+1)/\delta)}}{n^{3/2}}$ due to exploration to estimate the variances of each state-action pair.



\begin{customcorollary}{2}
The constraint regret of \sav\ is bounded by
$\cR^c_n \leq O\big(\frac{\log(n)}{n^{1/2}}\big)$ and the reward regret is bounded by $\cR_n \leq O\big(\frac{\log(n)}{n^{3/2}}\big)$.
\end{customcorollary}

The proof is in \Cref{app:mdp-regret-corollary} and directly follows from Thm \ref{thm:mdp-oracle-loss}, \ref{thm:mdp-agnostic-loss}. Observe, that the regret decreases at a rate of $O(n^{-3/2})$, faster than the rate of decrease of MSE of  $O(n^{-1})$. 



\begin{customcorollary}{2}
    Bandit Regret
\end{customcorollary}


% We do not have a regret lower bound for the Tree-MDP setting and we leave it to future work.

\textbf{Extension to DAG:} We define a DAG MDP $\G$ in \Cref{def:dag-mdp}. The \Cref{lemma:dag} \citep{mukherjee2022revar} shows that one cannot derive a closed-form solution to $\bb^*$ in $\G$ because of the existence of multiple paths to the same state resulting in the cyclical dependency. Note that in $\T$ there is a single path to each state and this cyclical dependency does not arise. However, we can approximate the optimal sampling proportion that ignores the multiple path problem in $\G$ by using the tree formulation. We state an iterative algorithm in \Cref{alg:revar-g-1} that uses value-iteration for the episodic setting \citep{sutton2018reinforcement} to estimate the optimal sampling proportion iteratively. This is shown in \Cref{app:dag}.

% and this is shown in \Cref{app:dag}.

==> oracle.tex <==
In this section, we consider the bandit setting consisting of a single state and finite action set $\A$. Hence we drop the state $s$ from our notation. For easier exposition to bandit literature, we will index the model parameters with time $\ell$ and drop the episode number $k$. So we have the time index $\ell\in[n]$.
%
%
We can restate the safety constraint \eqref{eq:safety-constraint-MDP} for the bandit setting as follows:
\begin{align}
    &\min_{\{\bb^{\ell'}\}_{\ell'=1}^n} \E_{\D}[(V_{\pi} - Y_n)^2 | A_{\ell'} \sim \bb^{\ell'}] \quad \text { s.t.} %\nonumber\\
    %%%%%%%%%%%%%%%
    \sum_{\ell'=1}^\ell \mu^c(A_{\ell'}) \geq(1-\alpha) \mu^c(0) \ell, 
    \text{ for all } \ell\in[n] \label{eq:safety-constraint-bandit}
\end{align}
with high probability, $A_{\ell'}$ is the action at $\ell'$, and $\{\bb^{\ell'}\}_{\ell'=1}^n$ is a sequence of time-dependent behavior policies. 
% We first discuss the oracle strategy for this setting. Again recall that 

\vspace*{-1em}
\subsection{Oracle Strategy with no Constraints}
To build the safe agnostic algorithm for DCPE we first study an oracle that knows the reward variances  of each of the arms $a\in\A$ in the unconstrained setting.
%
% (both reward and cost) $\sigma^{2}(a)$ and $\sigma^{c,(2)}$ of each of the arms $a\in\A$. 
The works of \citet{carpentier2011finite,carpentier2012minimax, carpentier2015adaptive, fontaine2021online, mukherjee2022revar} also study a similar type of oracle that knows the variances. 
%
We are interested in this type of oracle as in the unconstrained setting, sampling trajectories according to this oracle behavior policy minimize the MSE of the estimator of the target policy.
% expected reward as well as complies with \eqref{eq:safety-constraint-bandit}. 
%
We assume that the oracle does not know the reward means as otherwise there is no need to do a policy evaluation. 
% 
% We also assume that the oracle does not know the cost means as knowing the cost means trivializes satisfying the cost constraint.


% \smnote{Say why we assume that the oracle does not know the means.}
%
% problem-dependent parameters i.e. the mean of all the actions $\mu(a)$, their variances $\sigma^2(a)$, along with the target policy $\pi$. Again recall that we are interested in this type of oracle as sampling trajectories according to this oracle behavior policy minimizes the MSE of the estimator of the target policy's expected reward as well as comply with \eqref{eq:safety-constraint-bandit}. 
%

Suppose we have a budget of $n$ samples to divide between the actions and let $T_n(1), T_n(2), \ldots, T_n(A)$ be the number of samples allocated to actions $1, 2, \ldots, A$ at the end of $n$ rounds. Then the goal of the oracle is to estimate the optimal sampling  proportion $\bb\in\triangle(\A)$ such that it reduces the MSE $\E_{\D}\big[\left(Y_n - V_{\pi}\right)^{2}\big]$.
%
%
It can be shown that the optimal oracle sampling proportion for the unconstrained setting is given by $\bb^*_{safe}(a)\propto \pi(a)\sigma(a)$ 
% when all the actions are known to be safe (i.e., $\mu^c(a) \geq (1-\alpha)\mu^c(0)$ for all $a$) 
\citep{carpentier2011finite, carpentier2015adaptive, fontaine2021online,  mukherjee2022revar}.
%
% \rev \citep{mukherjee2022revar} or \mcucb\ \citep{carpentier2011finite} 
%
%
We restate the result in \Cref{prop:bandit} in \Cref{app:prev-result} for completeness. Intuitively, there is more uncertainty about the mean reward for actions with higher variance reward distributions. Selecting these actions more often is needed to offset higher variance. The optimal proportion also takes $\pi$ into account as a high variance mean reward estimate for one action can be acceptable if $\pi$ would rarely take that action.
%
%Note that sampling according to \cref{eq:bandit-optimal-prop} introduces unnecessary variance compared to deterministically selecting actions to match the optimal proportion.
% 
Since the variances are typically unknown, a number of works in the bandit community propose different approaches to estimate the variances for both basic bandits and several related extensions (without safety constraints) \citep{antos2008active, carpentier2011finite, carpentier2012minimax, carpentier2015adaptive, neufeld2014adaptive,mukherjee2022revar}.
%
%
%Add later
% Finally, note that incorporating variance-aware techniques has been studied in bandits \citep{audibert2009exploration, mukherjee2018efficient}. However, these works tend to focus on regret minimization, whereas we focus on MSE reduction.
% 
% However, none of these works address the fundamental challenge that safety constraints and MDPs bring -- action selection must account for both immediate variance reduction in the current state as well as variance reduction in future states visited. (have to incorporate this statement)
%

% We now introduce a few notations for the bandit setting. We define the confidence interval for action $a$ at time $\ell$ as
% \begin{align}
%     C_\ell(a) \coloneqq (2\eta + 4\eta^2)\sqrt{\dfrac{\log(A n(n+1)/\delta)}{T_\ell(a)}}.\label{eq:confidence-interval-bandit}
% \end{align}
% We define the cost gap as $\Delta^c(a) \coloneqq \mu^{c,*} - \mu^c(a)$ where $\mu^{c,*} = \max_a \mu^c(a)$. 
% % We also define the cost safety gap as $\Delta^{c, \alpha}(a) \coloneqq (1-\alpha)\mu^c(0) - \mu^c(a)$ as the safety gap and $\Delta^{c, (2),\alpha}(a) \coloneqq (\Delta^{c, \alpha}(a))^2$. 
%
%




% The oracle-safe version of \rev 
% % (abbreviated as \sav) 
% can be stated as follows: For each time $\ell=1,2,\ldots,n$
% \begin{align}
% % &\text{For each time $\ell=1,2,\ldots,n$}\nonumber\\
% %%%%%%%%%%%%%%
%     \hspace*{-1em}\text{Sample } A_\ell=\begin{cases}
%         \argmax_a\frac{\bb^*(a)}{T_\ell(a)} &\text{ if } \wZ_\ell \geq 0, \ell > \sqrt{n}\\
%         %%%%%%%%%%%%
%         \sim \pi_e &\text{ if } \wZ_\ell \geq 0 , \ell \leq \sqrt{n}\\
%         %%%%%%%%%%%%
%         0 &\text{ if } \wZ_\ell < 0 \label{eq:saver-oracle-sample}
%     \end{cases}
% \end{align}
% where $\bb^*(a) = \pi(a)\sigma(a)$, $\wZ_\ell = \sum_{\ell'=1}^\ell \underline{\wmu}^c_{\ell'}(A_{\ell'}) + \underline{\wmu}^c_{\ell}(J_{\ell}) - (1-\alpha)\ell\mu^c(0)$ is the safety budget as oracle does not know the means of the actions (both cost and reward). The $\wZ_\ell$ is lower confidence bound to the true safety budget $\sum_{s=1}^\ell \mu^c(I_s) \geq(1-\alpha) \mu^c(0) \ell$. 
% % \jsnote{Just noting for now that this paragraph could be revised for clarity (what is safety budget and what is purpose of lower bound). sm: Added a line}
% Here, $A_{\ell'}$ is the action sampled at time $\ell'$, $\underline{\wmu}^c_{\ell'}(A_{\ell'}) = \wmu^c_{\ell'}(A_{\ell'}) - C_{\ell'}(A_{\ell'})$ is the lower confidence bound to the empirical cost mean, and $J_\ell = \argmax_a \tfrac{\pi(a)\sigma(a) }{T_\ell(a)}$ is the action that the oracle can sample in the $\ell$-th time. 
% %
% %
% Hence, when $\wZ_\ell \geq 0$ the oracle follows the \rev oracle proportion $\bb^*$ when $\ell > \sqrt{n}$ or plays the exploration policy $\pi_e$ to build a good cost estimate of each $\mu^c(s,a)$. In this paper, we take $\pi_e$ as a uniform sampling procedure (see \Cref{rem:pi-e}). When the safety budget $\wZ_\ell < 0$ it falls back to the baseline policy and samples it to make the $\wZ_\ell$ positive again. The exploration policy $\pi_e$ is required to explore actions and get a good estimate of the cost means $\mu^c(a)$. 
% % and could be any explorative policy like UCB \citep{auer2002finite} or uniform sampling. 
% %
% % Hence, the oracle follows the \rev oracle proportion when the safety budget $\wZ_\ell \geq 0$, else when $\wZ_\ell < 0$ it falls back to the safe action and samples it to make the $\wZ_\ell$ positive again. 
% %
% % Also, observe that, for $\ell > \sqrt{n},$ the action selection rule ensures that the ratio $\bb^*(a)/T_{\ell}(a) \approx 1$.
% % 
% It is a deterministic action selection rule and thus avoids variance due to simply sampling from the optimal proportions $\bb^*(a)$ and ensuring safety constraint.
% %
% % Observe that the randomness in $Z_t$ comes from following the proportion $\bb$. Note that \srev\ also knows the true variances of each action, and further observe that this sampling rule is different than \Cref{thm:bandit-oracle}. 
% % In the following theorem, we show that the MSE of the oracle following the sample proportion in \eqref{eq:saver-oracle-sample}.



% % Before defining the oracle data collection strategy, we first recall that using the \Cref{assm:unbiased-MDP} on the data $\D$ collected over $n$ action-reward samples we can ensure that the 
% % %
% % % state an assumption on $\D$. 
% % % \begin{assumption}
% % % \label{assm:unbiased}
% % % \textbf{(Data collection)}
% % % We will only consider data collection strategies such that the data $\D$ collected over $n$ action-reward samples eventually contains at least one observation of each action for which $\pi(a)>0$.
% % % \end{assumption}
% % % \Cref{assm:unbiased} ensures that 
% % $Y_n$ is an unbiased estimator of $V_{\pi}$ so that reducing the MSE is equivalent to reducing the variance. 
% % %



% Now recall that using the \Cref{assm:unbiased-MDP} we can show that $Y_n$ is an unbiased estimator of $V_{\pi}$ so that reducing the MSE is equivalent to reducing the variance. 
% %
% The oracle knows the variance and follows the sampling proportion in \eqref{eq:saver-oracle-sample}. After $n$ rounds, let the oracle algorithm return the empirical estimate $\wmu_{n}(a)$ of all the actions. Now the MSE is defined as follows:
% \begin{align*}
% \E_{\D}&\big[\left(Y_n- V_\pi\right)^2\big]=\E_{\D}\big[\big(\sum_{a=0}^A \pi(a)(\wmu_{n}(a)-\mu(a))\big)^2\big]\\
% %%%%%%%%%%%%%
% &\overset{(a)}{=}\sum_{a=0}^A \pi(a)^2 \E_{\D}\big[\big(\wmu_{n}(a)-\mu(a)\big)^2\big] = \L_n(\pi)
% \end{align*}
% where, $(a)$ follows as observations of actions $a,a'$ are independent of each other in our setting and finally, we denote the MSE of an algorithm as  $\L_n(\pi)$. 
% %
% % 
% We define the predicted oracle constraint violation as $\C_n^\star(\pi) \coloneqq \sum_{\ell=1}^n\indic{\wZ_\ell < 0}$ when taking actions according to \eqref{eq:saver-oracle-sample}. Similarly define predicted agnostic constraint violation $\C_n(\pi) \coloneqq \sum_{\ell=1}^n\indic{\wZ_\ell < 0}$ when taking actions according to \eqref{eq:saver-agnostic-sample}.
% %
% Define the complexity parameter $H_* \!\!=\!\!\! \frac{1}{\alpha\mu(0)}\!\!\!\sum\limits_{a\in\A\setminus\{0\}}\!\!\pi(a)\sigma(a)|\min\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}|$ which we discuss in \Cref{rem:H}. Define $M \!\!\coloneqq\!\! \sum_a \pi(a)\sigma(a)$. 
% %
% %
% % Define $\Delta^{\alpha}(a) = (1-\alpha)\mu(0) - \mu(a)$ as the safety gap and $\Delta^{(2),\alpha}(a) = (\Delta^{\alpha}(a))^2$. We now derive the MSE of this oracle in \eqref{eq:saver-oracle-sample} and discuss its implications. 


% \begin{customtheorem}{1}\textbf{(informal)}
% \label{thm:bandit-oracle-loss}
%     The MSE of the oracle for $\frac{n}{\log(An(n+1)/\delta)} \geq 4A + \frac{A}{\Delta^{c,(2)}_{\min}} + \frac{1}{4 H_*^2}$ 
%     % and safety gap $-\sqrt{\frac{K}{n}}\leq \Delta^{\alpha}(a)\leq \sqrt{Kn}$ 
%     is bounded with probability $(1\!-\!\delta)$ as $\L^*_n(\pi) \leq O\big(\frac{M^2}{n} + \frac{H^2_* M^2}{n}\big)$.
%     % \begin{align*}
%         % $\L^*_n(\pi) \leq O\bigg(\underbrace{\frac{M^2}{n}}_{\substack{\textbf{Safe MSE,}\\\wZ_t \geq 0}} + \underbrace{\frac{H^2_* M^2}{n}}_{\substack{\textbf{Unsafe MSE,}\wZ_t < 0}} \bigg).$
%     % \end{align*}
%     % where $H_* = \frac{1}{\alpha\mu(0)}\sum_{a\in\A\setminus\{0\}}\pi(a)\sigma(a)|\min\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}|$ is the problem complexity parameter. 
%     The total predicted constraint violations is bounded with probability $(1\!-\!\delta)$ as
%     % \begin{align*}
%         $\C^*_n(\pi) \leq O\left(\frac{H_*n}{M}\right)$.
%     % \end{align*}
%     % with probability $(1-\delta)$.
% \end{customtheorem}

% % \begin{proof}\textbf{(Overview)} 
% \textbf{Proof (Overview)}:
% The proof technique differs from \citet{wu2016conservative, yang2021reduction, mukherjee2022revar}. We divide the total budget $n = n_f + n_u$ where $n_f$ are the samples allocated when safety budget $\wZ_n \geq 0$. The $n_f$ samples are also used by the exploration policy $\pi_e$ to ensure a good estimate of the cost means as stated in the event $\xi_{c,n}$ \eqref{eq:good-cost-event}. This is ensured by $\pi_e$ and noting that $n > A\log(1/\delta)/\Delta^{c,(2)}_{\min}$ which ensures sufficient samples for exploration for each $a$. The remaining samples from $n_f$ are allocated for reducing the MSE by sampling according to $\argmax_a(\bb^*(a)/T_\ell(a))$. We prove an upper and lower bound to $T_{n}(a)$ in \eqref{eq:oracle-6-1} and \eqref{eq:oracle-6-2} in step $5$. This is because $T_{n_f}(a) = T_n(a)$ for $a\in\A\setminus\{0\}$ as for $n_u$ samples oracle selects only action $0$. Finally using \Cref{lemma:wald-variance} we can bound the MSE for the duration $n_f$ for $a\in\A\setminus\{0\}$ in step $6$. Now for an upper bound to constraint violations, we use the gap $\Delta^{c,\alpha}(a)\coloneqq(1-\alpha) \mu^c(0)-\mu^c(a)$ to bound how much each $a\in\A\setminus\{0\}$ is underpulled and their pulls replaced by action $\{0\}$ weighted by $\pi(a)\sigma(a)$. This is captured by $H_*$ and the upper bound to violation is shown in step $7$. Finally, we also need a lower bound to constraint violations to bound the MSE for the duration when actions $a\in\A\setminus\{0\}$ are underpulled. This is shown in steps $8$ and $9$ where we equate the safety budget to $0$ to obtain a lower bound to $T_n(0)$. Combining everything in step $10$ gives the result. The proof is in \Cref{app:bandit-oracle-loss}. $\blacksquare$
% %
% % Using \Cref{assm:unbiased-MDP} we can show $Y_n$ is an unbiased estimator of $V_\pi$, and we can focus on the variance of $Y_n$. We can rewrite the variance of $Y_n$ in terms the sampling proportion $\bb(a) = T_n(a)/\sum_{a'=0}^A T_n(a')$. Now we incorporate the safety constraint such that \smnote{To be written}.
% % \end{proof}


% From \Cref{thm:bandit-oracle-loss} observe  that the first quantity is denoted as the safe MSE when the safety budget $\wZ_n \geq 0$ and scales as $M^2/n$. The second quantity is denoted as the unsafe MSE which is accumulated due to constraint violation ($\wZ_n < 0$) and sampling of the safe action $0$. Comparing the result of the \Cref{thm:bandit-oracle-loss} with \citet{carpentier2011finite} we have the additional quantity of
% % \begin{align*}
%     $\frac{H^2_*M^2}{n}$
% % \end{align*}
% where $H_*$ is the problem-dependent quantity. Also, observe that if all actions are safe then we have that $\L^*_n(\pi) = \frac{M^2}{n}$ which recovers the MSE of the oracle in \citet{carpentier2011finite}.

% % \textbf{Discussion on $H_*$:} 
% \begin{remark}\label{rem:H}
% The quantity $H_*$ signifies the total cost of maintaining the safety constraint by sampling action $0$ instead of sampling based on $\pi(a)\sigma(a)$. Observe that $\Delta^c(0)-\Delta^c(a) = \mu^c(a) - \mu^c(0)$. So $\min^+\{\Delta^c(a),\Delta^c(0)-\Delta^c(a)\}$ depends on how close is the action $a$ to the best cost action $ \mu^{*,c}$ or the baseline action $0$. Also observe that because of the $\min^+$ operator, this quantity cannot be $0$. Further, observe that the gap is weighted by $\pi(a)\sigma(a)$ signifying that actions with low variance and target probability contribute less to the constraint violation MSE. Finally, observe that higher risk setting $(\alpha \rightarrow 0)$ leads to higher $H_*$.
% \end{remark}









\subsection{Agnostic Bandit Algorithm with Safety Constraints}

In this section, we introduce the more realistic algorithm that does not know the mean and variances of the actions and has to comply with the safety constraint in \eqref{eq:safety-constraint-bandit}.
%
Intuitively, the agnostic algorithm can build a safety budget $\wZ_\ell$ as a metric for how safe it is to follow the $\bb^*_{safe}$ at round $\ell$. If $\wZ_\ell > 0$ it can follow $\bb^*_{safe}$, otherwise it can follow the baseline policy.
%
A key challenge in our setting is that the constraint mean (variance) can be different from the reward mean (variance). Therefore, while exploring with $\bb^*_{safe}$ the algorithm can get a good estimate of $\mu(a)$ and $\sigma^2(a)$, this may not yield a good estimate of $\mu^c(a)$ and $\sigma^{(2),c}(a)$.
%
Hence, the learner also needs to run an exploratory policy $\pi_x$ to additionally estimate $\mu^c(a)$ and $\sigma^{(2),c}(a)$.

We now define the individual component of the agnostic algorithm before formally stating it.  
%
Let the safety budget be $\wZ_\ell = \sum_{\ell'=1}^\ell \underline{\wmu}^c_{\ell'}(A_{\ell'}) + \underline{\wmu}^c_{\ell}(J_{\ell}) - (1-\alpha)\ell\mu^c(0)$ as it does not know the means of the actions (both cost and reward). The $\wZ_\ell$ is lower confidence bound to the true safety budget $\sum_{s=1}^\ell \mu^c(I_s) \geq(1-\alpha) \mu^c(0) \ell$ defined in \eqref{eq:safety-constraint-bandit}. 
%
Here, $A_{\ell'}$ is the action sampled at time $\ell'$, $\underline{\wmu}^c_{\ell'}(A_{\ell'}) = \wmu^c_{\ell'}(A_{\ell'}) - C_{\ell'}(A_{\ell'})$ is the lower confidence bound to the empirical cost mean and $J_\ell$ is the action selected at round $\ell$. The confidence interval width $C_{\ell'}(A_{\ell'})$ is defined in \eqref{eq:confidence-interval} (adapted to the bandit setting). Define the upper confidence bound on the empirical reward variance as $\overline{\wsigma}_\ell(a) \coloneqq \wsigma_\ell(a) + C_\ell(a)$, where $C_\ell(a)$ is defined in \eqref{eq:confidence-interval}. We define the empirical sampling proportion $\wb_\ell(a) \coloneqq \pi(a)\overline{\wsigma}_\ell(a)$. 
%
% and $J_\ell = \argmax_a \tfrac{\pi(a)\sigma(a) }{T_\ell(a)}$ is the action that the oracle can sample in the $\ell$-th time. 
%
%


We formally state the \textbf{Sa}fe \textbf{V}arianc\textbf{e} \textbf{R}eduction algorithm (abbreviated as \sav). 
% in \Cref{alg:bandit-track}. 
It takes as input the risk parameter $\alpha > 0$ and target policy $\pi$ and builds the dataset $\D$. At every timestep $\ell\in[n]$ \sav\ generates a sampling history $\H_\ell \coloneqq \{A_{\ell},R^k_\ell(A_{\ell}),C^k_\ell(A_\ell)\}$ by selecting $A_\ell$ according to the following rule:
\begin{align}
% &\text{For each time $\ell=1,2,\ldots,n$}\nonumber\\
%%%%%%%%%%%%%%
    \hspace*{-1em}\text{Sample } A_\ell =\begin{cases}
        \argmax_a\frac{\wb_\ell(a)}{T_\ell(a)} &\text{ if } \wZ_\ell \geq 0, \ell > \sqrt{n}\\
        %%%%%%%%%%%%
        \sim \pi_x &\text{ if } \wZ_\ell \geq 0, \ell \leq \sqrt{n}\\
        %%%%%%%%%%%%
        0 &\text{ if } \wZ_\ell < 0 \label{eq:saver-agnostic-sample}
    \end{cases}
\end{align}
It then appends sampling history $\H_\ell$ to the dataset $\D$. Finally, it returns the dataset $\D$ to evaluate $\pi$.

We now briefly discuss the implication of the bandit \sav\ in \eqref{eq:saver-agnostic-sample}. When $\wZ_\ell \geq 0$ the oracle follows the $\bb^*_{safe}$ when $\ell > \sqrt{n}$ or plays the exploration policy $\pi_x$ to build a good cost estimate of each $\mu^c(s,a)$. 
%
We discuss the exploratory policy $\pi_x$ in \Cref{rem:pi-e}. 
%
% In this paper, we take $\pi_e$ as a uniform sampling procedure (see \Cref{rem:pi-e}). 
%
When the safety budget $\wZ_\ell < 0$ it falls back to the baseline policy (action $0$) and samples it to make the $\wZ_\ell$ positive again. Finally note that $\argmax_a\tfrac{\wb_\ell(a)}{T_\ell(a)}$
is a deterministic action selection rule and thus avoids variance due to simply sampling from the optimal proportions $\bb^*_{safe}(a)$ and ensuring safety constraint.
%
%
% Hence, when $\wZ_\ell \geq 0$ the oracle follows the $\bb^*_{safe}$ when $\ell > \sqrt{n}$ or plays the exploration policy $\pi_x$ to build a good cost estimate of each $\mu^c(s,a)$. In this paper, we take $\pi_e$ as a uniform sampling procedure (see \Cref{rem:pi-e}). When the safety budget $\wZ_\ell < 0$ it falls back to the baseline policy and samples it to make the $\wZ_\ell$ positive again. The exploration policy $\pi_e$ is required to explore actions and get a good estimate of the cost means $\mu^c(a)$. 
% and could be any explorative policy like UCB \citep{auer2002finite} or uniform sampling. 
%
% Hence, the oracle follows the \rev oracle proportion when the safety budget $\wZ_\ell \geq 0$, else when $\wZ_\ell < 0$ it falls back to the safe action and samples it to make the $\wZ_\ell$ positive again. 
%
% Also, observe that, for $\ell > \sqrt{n},$ the action selection rule ensures that the ratio $\bb^*(a)/T_{\ell}(a) \approx 1$.
% 
% It is a deterministic action selection rule and thus avoids variance due to simply sampling from the optimal proportions $\bb^*(a)$ and ensuring safety constraint.
%
% Observe that the randomness in $Z_t$ comes from following the proportion $\bb$. Note that \srev\ also knows the true variances of each action, and further observe that this sampling rule is different than \Cref{thm:bandit-oracle}. 
% In the following theorem, we show that the MSE of the oracle following the sample proportion in \eqref{eq:saver-oracle-sample}.
%
%
%
% but samples according to optimal oracle sampling rule $\bb^*_{safe}(a)\propto \pi(a)\sigma(a)$ when 
%
%
%
% in \eqref{eq:saver-oracle-sample}. We then analyze this algorithm and establish its regret bound against the MSE of the oracle derived in \Cref{thm:bandit-oracle-loss}. 
%
% We introduce a few notations before presenting the algorithm. Define the upper confidence bound on the empirical reward variance as $\overline{\wsigma}_\ell(a) \coloneqq \wsigma_\ell(a) + C_\ell(a)$, where $C_\ell(a)$ is defined in \eqref{eq:confidence-interval}. We define the empirical sampling proportion $\wb_\ell(a) \coloneqq \pi(a)\overline{\wsigma}_\ell(a)$. Finally, 
%
%
%
% We formally state the \textbf{Sa}fe \textbf{V}arianc\textbf{e} \textbf{R}eduction algorithm (abbreviated as \sav). 
% % in \Cref{alg:bandit-track}. 
% It takes as input the risk parameter $\alpha > 0$ and target policy $\pi$ and builds the dataset $\D$. At every timestep $\ell\in[n]$ \sav\ generates a sampling history $\H_\ell \coloneqq \{A_{\ell},R^k_\ell(A_{\ell}),C^k_\ell(A_\ell)\}$ by selecting $A_\ell$ according to \eqref{eq:saver-agnostic-sample} and appends it to the dataset $\D$. 
% %
% After observing the feedback \sav\ updates the model parameters and estimate $\wb^{}_{\ell+1}(a)$ for each action $a$. Finally, it returns the dataset $\D$ to evaluate $\pi$. This full pseudocode is shown in \Cref{alg:bandit-track}.
% \begin{algorithm}
% \caption{\textbf{Sa}fe \textbf{V}arianc\textbf{e} \textbf{R}eduction (\sav) for Bandit}
% \label{alg:bandit-track}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Risk Parameter $\alpha>0$, target policy $\pi$.
% \State \textbf{Output:} Dataset $\D$.
% \State Initialize $\D = \emptyset$, $\wb^{}_1(a)$ uniform over all actions.
% \For{$\ell=1,2,\ldots,n$}
% \State Generate history $\H_\ell \coloneqq \{A_{\ell},R^k_\ell(A_{\ell}),C^k_\ell(A_\ell)\}$ by selecting \indent$A_\ell$ according to \eqref{eq:saver-agnostic-sample}.
% \State $\D \leftarrow \D \cup \{(\H_\ell, \wb_\ell)\}$
% \State Update model parameters and estimate $\wb^{}_{\ell+1}(a)$ for \indent each $a$ such that $\wb_{\ell+1}(a) \coloneqq \pi(a)\overline{\wsigma}_{\ell+1}(a)$. 
% % \State Update $\wb^{}_{\ell}(a)$ following \eqref{eq:bandit-bhat} for each action $a$ .
% \EndFor
% \State \textbf{Return} Dataset $\D$ to evaluate policy $\pi$.
% \end{algorithmic}
% \end{algorithm}
%
% 
We present the MSE of the \sav\ in the following theorem.


\begin{customtheorem}{1}\textbf{(informal)}
\label{thm:bandit-agnostic-loss}
    The MSE of the bandit \sav\ following for $\tfrac{n}{\log(An(n+1)/\delta)} \geq 4A  + \tfrac{A}{\Delta^{c,(2)}_{\min}} + \tfrac{1}{4 H_*^2}$ 
    % and safety gap $-\sqrt{\frac{K}{n}}\leq \Delta^{\alpha}(a)\leq \sqrt{Kn}$ 
    is bounded w.p. $(1\!-\!\delta)$ as $\L_n(\pi) \leq O\big(\tfrac{M^2}{n} + 
        \tfrac{\sqrt{\log (A n(n+1)/\delta)}}{\bb_{\min}^{3/2}n^{3/2}} + 
        \tfrac{H^2_* M^2}{n} \big)$.
    % \begin{align*}
    %     &\L_n(\pi) \leq O\bigg(\underbrace{\frac{M^2}{n}}_{\substack{\textbf{Safe Loss,}\\\wZ_t \geq 0}} + 
    %     \underbrace{\dfrac{\sqrt{\log (A n(n+1)/\delta)}}{\bb_{\min}^{3/2}n^{3/2}}}_{\substack{\textbf{Exploration Loss}}} + 
    %     % \\
    %     %%%%%%%%%%%%%
    %     \underbrace{\dfrac{H^2_* M^2}{n}}_{\substack{\textbf{Unsafe Loss,}\\\wZ_t < 0}} \bigg).
    % \end{align*}
    % where $H_* = \sum_{a\in\A\setminus\{0\}}\frac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}$ is the problem complexity parameter. 
    The total predicted constraint violations are bounded as
    % \begin{align*}
        $\C_n(\pi) \leq O\big(\frac{H_* n}{M} + \frac{\sqrt{\log (A n(n+1)/\delta)}}{n^{1/2}}\big)$
    % \end{align*}
    % with probability $(1-\delta)$.
    w.p. $(1\!-\!\delta)$.
\end{customtheorem}

% \begin{proof}\textbf{(Overview)}
\textbf{Proof (Overview)}
    Note that \sav\ does not know the reward variances. The sampling rule in \eqref{eq:saver-agnostic-sample} ensures that the good variance event $\xi_{v,n}$ in \eqref{eq:bandit-good variance-event} holds such that \sav\ has good estimates of reward variances. The remaining  
    proof follows the same steps as \Cref{thm:bandit-oracle-loss} where we plug-in the upper bound to $\sigma(a)$. The proof is in \Cref{app:bandit-saver-loss}. $\blacksquare$
% \end{proof}

From the result of \Cref{thm:bandit-agnostic-loss} we can show that the agnostic \sav\ suffers an additional MSE factor that scales as $\frac{\sqrt{\log (A n(n+1)/\delta)}}{\bb^{3/2}_{\min} n^{3/2}}$ due to exploration to estimate the variances of each action. We now define two notions of regret. The first is the constraint regret defined as follows:
% \begin{align}
    $\cR^c_n = \C_n - \overline{\C}^*_n$ 
    % \label{eq:bandit-constraint-regret}
% \end{align}
where, $\overline{\C}^*_n$ is the upper bound to the oracle constraint violations.
% where, $\C_n = \sum_{\ell=1}^n\indic{\wZ_t < 0, A_\ell\sim \{\wb_t, \pi_0\}}$ is the number of times the constraint is violated following $\wb_t$ and $\C^*_n = \sum_{\ell=1}^n\indic{\wZ_\ell < 0, A_\ell\sim \{\bb^*, \pi_0\}}$ is the constraint violation of the oracle.
The second is the reward regret defined as 
% \begin{align}
    $\cR_n = \L_n(\pi) - \overline{\L}^*_n(\pi)$ %\label{eq:bandit-reward-regret}
% \end{align}
where $\overline{\L}^*_n(\pi)$ is the upper bound to the oracle MSE. Note that we consider an upper bound of the oracle MSE as well as constraint violations because we do not have a closed-form solution to $\bb^*$ that both minimizes MSE as well as upholds \eqref{eq:safety-constraint-MDP} for all $k\in[K]$ (as opposed to \citet{carpentier2011finite, mukherjee2022chernoff}). The following corollary bounds \sav\ regret.
\begin{customcorollary}{1}
The constraint regret of \sav\ is bounded by
$\cR^c_n \leq O\big(\frac{\log(n)}{n^{1/2}}\big)$ and the reward regret is bounded by $\cR_n \leq O\big(\frac{\log(n)}{n^{3/2}}\big)$ in the bandit setting.
\end{customcorollary}

The proof is in \Cref{app:bandit-regret-corollary} and directly follows from Thm \ref{thm:bandit-oracle-loss}, \ref{thm:bandit-agnostic-loss}. Observe, that the regret decreases at a rate of $O(n^{-3/2})$, faster than the rate of decrease of MSE of  $O(n^{-1})$. In \Cref{thm:bandit-lower-bound} in \Cref{app:bandit-lower-bound} we show a bandit regret lower bound and discuss its implications in \Cref{rem:comparing-regret}. 

==> oracle_proof.tex <==
% \subsubsection{Support Lemma}

% \begin{lemma}
% \label{lemma:conc}
% This lemma bounds the good variance event 
% \begin{align}
% \xi_{v,t}(\delta)=\left(\bigcap_{1 \leq a \leq A, 1\leq T_t(a) \leq t}\left\{\left|\frac{1}{T_t(a)}\sum_{t'=1}^{T_t(a)} R_{t'}^{2}(a)-\mu^{2}(a)\right| \leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right) \bigcap \nonumber\\
% %%%%%%%%%%%%%%%%%%%%%
% \left(\bigcap_{1 \leq a \leq A, 1\leq T_n(a) \leq \ell}\left\{\left|\frac{1}{T_t(a)}\sum_{\ell'=1}^{T_n(a)} R_{\ell'}(a)-\mu(a)\right| \leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right)\label{eq:event-xi-variance}
% \end{align}
% Then we can show that $\sum_{\ell=1}^n\Pb\left(\xi_{v,\ell}(\delta)\right) \geq 1- 2n\delta$.
% \end{lemma}





% %%%%%%%%%% Conc Lemma %%%%%%%%%%%%
% \input{conc_lemma}

% \begin{lemma}
% Let the empirical safety set at timestep $\ell$ be defined as $\wA_{s,\ell}$. Then on the event $\xi_{s,\ell}$ a safe action $a\in\sA$ and in $\wA_{s,\ell}$ is bounded as follows:
% \begin{align*}
%     \sum_{\ell=1}^n\Pb\left(a\in \wA_{s,\ell}\cap\sA \right) \geq 1 - n\delta.
% \end{align*}
% Similarly on the event $\xi_s$ an unsafe action $a\in\uA$ and in the empirical unsafe set $\wA_{u,\ell}$ is given by
% \begin{align*}
%     \sum_{\ell=1}^n\Pb\left(a\in \wA_{u,\ell}\cap\uA \right) \geq 1 - n\delta.
% \end{align*}
% % set at timestep $\ell > 4A$ and under the event $\xi_s$ is bounded by
% % \begin{align*}
% %     \Pb\left(\wA_{s,\ell}\neq \A_s\right) \leq 
% % \end{align*}
% \end{lemma}

% \begin{proof}
% Recall that the good safety event $\xi_{s,\ell}$ such that 
% \begin{align*}
% \xi_{s,\ell}(\delta)=\bigcap_{1 \leq a \leq A, 1 \leq T_t(a) \leq \ell}\left\{\left|\frac{1}{T_t(a)}\sum_{\ell'=1}^{T_t(a)} R_{\ell'}(a)-\mu(a)\right| \leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}
% \end{align*}
% So at $\xi_{s,\ell}$ it follows then that
% \begin{align*}
%     \mu(a) \geq \wmu_t(a) - (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}
% \end{align*}
% Now recall that a action $a\in\A$ is in the empirical safety set $\wA_{s,\ell}$ if
% \begin{align*}
%     &\wmu_t(a) - (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_n(a)}} \geq (1-\alpha)\mu(0) %\\
%     %%%%%%%%%%%%%%%%
%     \implies \mu(a) \geq (1-\alpha)\mu(0).
%     % \implies &\wmu_t(a) - \frac{(2\eta + 4\eta^2)}{2} \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_n(a)}} \geq (1-\alpha)\mu(0) - \frac{(2\eta + 4\eta^2)}{2} \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_n(a)}}. 
% \end{align*}
% By the definition of our safe action such that if an action $a$ is in $\sA$ we have that
% \begin{align*}
%     (1-\alpha)\mu(0) \leq \mu(a)
% \end{align*}
% Hence, under the safety set $\xi_{s,\ell}$ we have the true safe action $a\in\sA$ also in $\wA_{s,\ell}$ with the same probability as $\Pb(\xi_{s,\ell})$. Hence, union bounding over all $\ell\in[n]$ we have that $\sum_{\ell=1}^n\Pb\left(a\notin \wA_{s,\ell}\cap\A_{s} \right) \leq n\delta$
% \end{proof}
    



% \begin{lemma}
% Define the quantity $\Delta(a) = (1-\alpha)\mu(0) - \mu(a)$ and empirical estimate $\wDelta_t(a) = (1-\alpha)\mu(0) - \wmu_t(a)$. Then define
% \begin{align*}
%     B_s &= \sqrt{\sum_{a\in\sA}\pi^2(a)\sigma^2(a)\Delta^2(a)}, \wB_{s,\ell} = \sqrt{\sum_{a\in\sA}\pi^2(a)\wsigma^2_t(a)\wDelta^2_t(a)},\\
%     %%%%%%%%%%%%%%%%%%%%%%%
%     B_u &= \sqrt{\sum_{a\in\uA}\pi^2(a)\sigma^2(a)\Delta^2(a)}, \wB_{u,\ell} = \sqrt{\sum_{a\in\uA}\pi^2(a)\wsigma^2_t(a)\wDelta^2_t(a)}.
% \end{align*}
% Then under the event $\xi_{s,\ell}(\delta)\cap\xi_{v,\ell}(\delta)$ we have that
% \begin{align*}
%     &\sum_{\ell=1}^n\Pb\left(\left|\wB_{s,\ell} - B_s\right| < (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 \ell}}\right)\geq 1 - 4n\delta\\
%     %%%%%%%%%%%%%%%%
%     &\sum_{\ell=1}^n\Pb\left(\left|\wB_{u,\ell} - B_u\right| < (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2t}}\right)\geq 1 - 4n\delta.
% \end{align*}
% \end{lemma}


% \begin{proof}
% We will first try to bound $\sum_{a\in\A_s}\Delta^2(a) = (1-\alpha)\mu(0) - \mu(a)$ with respect to $\sum_{a\in\wA_{s,\ell}}\wDelta^2_t(a) = (1-\alpha)\mu(0) - \wmu_t(a)$, where $\wA_{s,\ell}$ is the set of safe actions in the empirical safety set. We now focus on the quantity
% \begin{align*}
%     \Delta^2(a) - \wDelta^2_t(a) &= \left((1-\alpha)\mu(0) - \mu(a)\right)^2 - \left((1-\alpha)\mu(0) - \wmu_t(a)\right)^2\\
%     %%%%%%%%%%%%%%%%%%%%%%%%
%     &\overset{(a)}{=} \left(b - \mu(a)\right)^2 - \left(b - \wmu_t(a)\right)^2\\
%     %%%%%%%%%%%%%%%%%%%%%%
%     &\overset{(a)}{=} \left(b^2 +  \mu^2(a) - 2b\mu(a)\right) - \left(b^2 + \wmu^2_t(a) - 2b\wmu_t(a)\right)\\
%     %%%%%%%%%%%%%%%%%%%%%%
%     &= 2b\left(\wmu_t(a) - \mu(a)\right) - \left(\wmu^2_t(a) - \mu^2(a)\right)
% \end{align*}
% where, $(a)$ follows for $b=(1-\alpha)\mu(0) $. This implies that
% \begin{align*}
%     \left|\Delta^2(a) - \wDelta^2_t(a)\right| = \left|2b\left(\wmu_t(a) - \mu(a)\right) - \left(\wmu^2_t(a) - \mu^2(a)\right)\right| \leq 2b\left|\wmu_t(a) - \mu(a)\right| + \left|\wmu^2_t(a) - \mu^2(a)\right|
% \end{align*}
% Now under the event $\xi_{s,\ell}(\delta)\cap\xi_{v,\ell}(\delta)$ observe that we have for each action $a$ the following
% \begin{align*}
%     &\Pb\left(\bigcap_{a\in\sA, 1\leq T_t(a) \leq \ell}\left\{|\wmu_t(a) - \mu(a)|\right\}\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right)\leq \delta/A\\
%     %%%%%%%%%%%%%%%
%     &\Pb\left(\bigcap_{a\in\sA, 1\leq T_t(a) \leq \ell}\left\{|\wmu^2_t(a) - \mu^2(a)|\right\}\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right) \leq \delta/A.
% \end{align*}
% from \Cref{lemma:conc1}. Then it follows that
% \begin{align*}
%     \Pb\left(\bigcap_{a\in\sA, 1\leq T_t(a) \leq \ell}\left\{\left|\Delta^2(a) - \wDelta^2_t(a)\right|\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right) \leq 2\delta/A
% \end{align*}
% Finally union bounding over all rounds $\ell\in[n]$ and actions in $\sA$ and noting that $|\sA| \leq |\A|$ we have that
% \begin{align}
%     \sum_{\ell=1}^n\Pb\left(\bigcap_{a\in\sA, 1\leq T_t(a) \leq \ell}\left\{\left|\Delta^2(a) - \wDelta^2_t(a)\right|\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right) \leq 2n\delta. \label{eq:B-1}
% \end{align}
% Similarly for the unsafe actions observe that under the event $\xi_{u,\ell}(\delta)\cap\xi_{v,\ell}(\delta)$ and
% % observe that we have for each action $a$ the following
% % \begin{align*}
% %     &\Pb\left(\bigcap_{1\leq T_t(a) \leq \ell}\left\{|\wmu_t(a) - \mu(a)|\right\}\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right)\leq \delta/A\\
% %     %%%%%%%%%%%%%%%
% %     &\Pb\left(\bigcap_{1\leq T_t(a) \leq \ell}\left\{|\wmu^2_t(a) - \mu^2(a)|\right\}\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right) \leq \delta/A.
% % \end{align*}
% using \Cref{lemma:conc} we have that
% \begin{align*}
%     \Pb\left(\bigcap_{a\in\uA, 1\leq T_t(a) \leq \ell}\left\{\left|\Delta^2(a) - \wDelta^2_t(a)\right|\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right) \leq 2\delta/A
% \end{align*}
% Finally union bounding over all rounds $\ell\in[n]$ and actions in $\uA$ and noting that $|\uA| \leq |\A|$ we have that
% \begin{align}
%     \sum_{\ell=1}^n\Pb\left(\bigcap_{a\in\uA, 1\leq T_t(a) \leq \ell}\left\{\left|\Delta^2(a) - \wDelta^2_t(a)\right|\geq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right) \leq 2n\delta. \label{eq:B-2}
% \end{align} 
% Also recall that we have from \Cref{corollary:conc} that with probability greater than $(1-2n\delta)$
% \begin{align}
%     \sum_{\ell=1}^n|\wsigma^{}_t(a) - \sigma(a)|\leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(s,a)}}. \label{eq:B-3}
% \end{align}

% Now observe that under $\xi_{s,\ell}$, we have $\wA_{s,\ell} \subseteq \sA$ with high probability. Then
% \begin{align*}
%     |\wB_{s,\ell} - B_s| = \left|\sqrt{\sum_{a\in\sA}\pi^2(a)\wsigma^2_t(a)\wDelta^2_t(a)} - \sqrt{\sum_{a\in\sA}\pi^2(a)\sigma^2(a)\Delta^2(a)}\right| &\overset{(a)}{\leq} \left|\sum_{a\in\sA}\left(\Delta^2(a) - \wDelta^2_t(a)\right)\right| +  \left|\sum_{a\in\sA}\left(\sigma^2(a) - \wsigma^2_t(a)\right)\right|\\
%     %%%%%%%%%%%%%%%
%     &\overset{}{\leq} \sum_{a\in\sA}\left|\left(\Delta^2(a) - \wDelta^2_t(a)\right)\right| +  \sum_{a\in\sA}\left|\left(\sigma^2(a) - \wsigma^2_t(a)\right)\right|
% \end{align*}
% where, $(a)$ follows for any $a,b > 0$ we have that $|a - b| \leq |a^2 - b^2|$. Let
% \begin{align*}
%     C_t = (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 \ell}}
% \end{align*}
% Then observe that under the condition that $\ell \geq T_t(a)$ and $|\sA|\geq 1$ we have that
% \begin{align*}
%     \sum_{a\in\sA}(2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}} > (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}} \overset{(a)}{>} (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 \ell}} = C_t
% \end{align*}
% where, $(a)$ follows for the condition that $\ell \geq T_t(a)$. A similar observation holds for 
% \begin{align*}
%     \sum_{a\in\uA}(2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}} > (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 \ell}} = C_t
% \end{align*}
% Using \Cref{eq:B-1}, \Cref{eq:B-2} and \Cref{eq:B-3} and union bounding over each action $a\in\sA$ and $a\in\uA$ it follows then that 
% \begin{align*}
%     \sum_{\ell=1}^n\Pb\left(\left\{\left|\wB_{s,\ell} - B_s\right|\geq \sum_{a\in\sA}(2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right)\overset{(a)}{\leq} \sum_{\ell=1}^n\Pb\left(\left\{\left|\wB_{s,\ell} - B_s\right|\geq C_t\right\}\right) \leq 4n\delta\\
%     %%%%%%%%%%%%%%%%%
%     \sum_{\ell=1}^n\Pb\left(\left\{\left|\wB_{u,\ell} - B_u\right|\geq \sum_{a\in\uA}(2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\}\right)\overset{(b)}{\leq} \sum_{\ell=1}^n\Pb\left(\left\{\left|\wB_{u,\ell} - B_u\right|\geq C_t\right\}\right) \leq 4n\delta
% \end{align*}
% where, $(a)$ and $(b)$ follows by noting that the probability of crossing a smaller threshold is larger. 
% The claim of the lemma follows.
% \end{proof}



% \jsnote{From here to Theorem 1 is just scratch work from our meeting, right?}
% Constrained Policy Evaluation in Bandits
% \begin{align*}
%     \min^{+}_\textbf{b} \E_{\D}[(v(\pi) - Y_n)^2 | I_s \sim b_s] \quad \text { s.\ell.} \sum_{s=1}^\ell \mu^c_{I_s} \geq(1-\alpha) \mu^c_0 \ell \quad \text { for all } \ell \in\{1, \ldots, n\}
% \end{align*}
% the $\textbf{b}$ is a sequence of time-dependent behavior policies. 

% It's possible that $\mu^r(a) \neq \mu^c(a)$. This implies that we need to keep an estimate of both $\wmu^r_t(a)$, $\wsigma^r_t(a)$, $\wmu^c_t(a)$, $\wsigma^c_t(a)$. The oracle knows the $\mu^c(a)$ and $\sigma^r(a)$. 

% Constrained Policy Evaluation in MDPs
% \begin{align*}
%     \min^{+}_\textbf{b} \E_{\D}[(v(\pi) - Y_n(s_0))^2] \quad \text { s.\ell.} \sum_{m=1}^k V_{b_m}^c \geq (1-\alpha) V^c_0 k \quad \text { for all } k \in\{1, \ldots, K\}
% \end{align*}
% where $s_0$ is the initial state, and $k$ is the number of episodes. The constraint now we have that
% \begin{align*}
%     % \sum_{s=1}^k V_{b_s}^c \coloneqq \sum_{s=1}^k\sum_{a}\bb^s(a|s_1)\left(\mu^c(s_1,a) + \sum_{s'}P(s'|s,a)\sum_{a'}\bb^s(a'|s')\mu^c(s',a)\right) \geq (1-\alpha) V^c_0 k\\
%     %%%%%%%%%%%%
%     \sum_{m=1}^k V_{b_m}^c(s_1) \coloneqq \sum_{m=1}^k\sum_{a}\bb^m(a|s_1)\left(\mu^c(s_1,a) + \sum_{s'}P(s'|s_1,a) V_{b_m}^c(s')\right) \geq (1-\alpha) V^c_0 k %\label{eq:safety-constraint-MDP}
% \end{align*}
% for all $k \in\{1, \ldots, K\}$.




% \begin{align*}
% \sum_{s=1}^\ell \mu_{I_s} \geq(1-\alpha) \mu_0 \ell \quad \text { for all } \ell \in\{1, \ldots, n\}
% \end{align*}


% Wu et al.
% \begin{align*}
%     \min^{+} R_n \quad \text { s.\ell.} \sum_{s=1}^\ell \mu^c_{I_s} \geq(1-\alpha) \mu^c_0 \ell \quad \text { for all } \ell \in\{1, \ldots, n\}
% \end{align*}

% \begin{align*}
% \min^{+}_\pi V_r^\pi(\rho) \quad \text { s.\ell. } \quad V_c^\pi(\rho) \geq \tau
% \end{align*}

% Vaswani (for bandits)
% \begin{align*}
% \min^{+}_\pi \sum_a \pi(a) \mu_r(a) \quad \text { s.\ell. } \quad \sum_a \pi(a) \mu_c(a) \geq \tau
% \end{align*}




% \begin{lemma}
% \label{lemma:bound-pulls}
% Let $n\geq 4A$ and $c>0$. Then we can show that
% \begin{align*}
%     T^*_n(p) &- 24\bb(p) (c + M B_s)  \frac{\sqrt{n\log (2 / \delta)}}{M \bb_{\min^{+}}^{3 / 2}}-8\bb(p)A \leq T_n(p) \leq T^*_n(p) + 24 (c + M B_s) \frac{\sqrt{n\log (2 / \delta)}}{M \bb_{\min^{+}}^{3 / 2}} + 8A, \textbf{ if $p\in\sA$}\\
%     %%%%%%%%%%%%%%%%%%%%%%
%     T^*_n(p) &- 24\bb(p) (c + M B_s) \frac{\sqrt{n\log (2 / \delta)}}{M \bb_{\min^{+}}^{3 / 2}}-8\bb(p)A \leq T_n(p) \leq T^*_n(p) + 24 (c + M B_u) \frac{\sqrt{n\log (2 / \delta)}}{M \bb_{\min^{+}}^{3 / 2}} + 8A, \textbf{ if $p\in\uA$}\\
%     %%%%%%%%%%%%%%%%%%%%%%%
%     T_n(0) &\leq \frac{2 A+2}{\alpha \mu(0)}+\frac{1}{\alpha \mu(0)} \sum_{a\in\uA}^A \dfrac{2\log(2/\delta)}{\Delta(a)}\left(\dfrac{\pi(a)\sigma(a)}{M B_u}n + 32 (c + M B_u) \frac{\sqrt{n\log (2 / \delta)}}{M \bb_{\min^{+}}^{3 / 2}}\right) \nonumber\\
%     %%%%%%
%     &\qquad+ \frac{1}{\alpha \mu(0)}\sum_{a\in\sA\setminus\{0\}}\dfrac{2\log(2/\delta)}{\Delta(0)-\Delta(a) }\left(\dfrac{\pi(a)\sigma(a)}{M B_s}n + 32 (c + M B_s) \frac{\sqrt{n\log (2 / \delta)}}{M \bb_{\min^{+}}^{3 / 2}}\right)
% \end{align*}
% \end{lemma}



\begin{customtheorem}{1}\textbf{(formal)}
    The MSE of the oracle for $\frac{n}{\log(An(n+1)/\delta)} \geq 4A + \frac{A}{\min_{a}\Delta^{c,(2)}(a)} + \frac{1}{4 H^2_*}$ is bounded by
    \begin{align*}
        \L^*_n(\pi) \leq \frac{M^2}{n}+\frac{16A M^2}{n^2} + \frac{16A^2 M^2}{n^3} + \dfrac{M^2A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + \dfrac{2}{n}.
    \end{align*}
    with probability $(1-\delta)$. The $H_* = \frac{1}{\alpha\mu(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta(a),\Delta(0)-\Delta(a) \}\pi(a)\sigma(a)$ is the problem complexity parameter. The total predicted constraint violations is bounded by
    \begin{align*}
        \C^*_n(\pi) \leq \dfrac{H_* n}{2 M}
        %
        % \frac{1}{2\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\min\{\Delta(a),\Delta(0)-\Delta(a) \}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)
        % \frac{2 A+2}{\alpha \mu(0)}+\frac{2\log(An(n+1)/\delta)}{\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\min\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)
    \end{align*}
    with probability $(1-\delta)$.
\end{customtheorem}

% \smnote{Oracle knows only the variance, but not the means.}

\begin{proof}
\textbf{Step 1 (Sampling rule):} First note that oracle samples by the following rule
\begin{align}
    A_\ell = \begin{cases}  \argmax_{a\in\A}\bigg\{\dfrac{\pi(a)\sigma(a)}{T_{\ell}(a)}\bigg\}, &\text{ if } \wZ_{\ell} \geq 0, \ell > \sqrt{n}\\
    %%%%%%%%%%%%%
    \sim \pi_e, &\text{ if } \wZ_{\ell} \geq 0, \ell \leq \sqrt{n} \\
    %%%%%%%%%%%%%
    0 &\text{ if } \wZ_{\ell} < 0 
    \end{cases} \label{eq:bandit-sampling-rule-1}.
\end{align}
where, $\wZ_\ell = \left(\sum_{\ell'=1}^{\ell-1}\wmu^c_{\ell'}(A_{\ell'}) - C_{\ell'}(A_{\ell'})\right) + \left(\wmu^c_{\ell}(J_\ell) - C_\ell(J_\ell)\right) - (1-\alpha)\ell\mu^c(0)$ is the safety budget and $J_\ell = \argmax_a\frac{\pi(a)\sigma(a)}{T_{\ell}(a)}$. The exploration policy $\pi_e$ is a uniform sampling procedure (see \Cref{rem:pi-e}), that results in the good cost estimate of actions as defined in \eqref{eq:good-cost-event}. This is proved in \Cref{corollary:safe-conc}.

\textbf{Step 2 (MSE Decomposition):} Also recall that the oracle knows the variances but does not know the means (cost and reward). We define the good cost event when the oracle has a good estimate of the cost mean. This is stated as follows:
\begin{align}
    \xi_{c,n} = \bigcap_{\substack{1\leq \ell \leq n,\\ 1\leq a \leq A}}\left\{\left|\wmu^c_t(a)-\mu^c(a)\right|\leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right\} \label{eq:good-cost-event}
\end{align}
Define $c_1 = 2\eta + 4\eta^2$. We also define the safety budget event
\begin{align*}
    \xi_{Z,n} = \bigcap_{1\leq \ell \leq n}\left\{\wZ_{\ell} \geq 0\right\}.
\end{align*}
Now using \Cref{lemma:wald-variance} we can show that 
\begin{align*}
    \sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{Z,n}}\cap\indic{\xi_{c,n}}\right] \leq \sum_{a\in\A}  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right]}{\underline{T}^2_{n}(a)}
\end{align*}
which implies that the oracle does not need to know the reward means $\mu(a)$. Hence, Using the definition of MSE we can show that the MSE of oracle is bounded by
\begin{align*}
\L_n(\pi) 
% &\leq \sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{s,n}\cap\xi_{v,n}\}\right] + \sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{v,n}^C\}\right] \\
%%%%%%%%%%%%%%
% &\qquad + \sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{s,n}^C\}\right] \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{Z,n}}\cap\indic{\xi_{c,n}}\right]}_{\textbf{Part A, $\wZ_n \geq 0$, safety event holds}}%\\
%%%%%%%%%%%%%
+ \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi^C_{Z,n}}\right]}_{\textbf{Part B, $\wZ_n < 0$, constraint violation}} \\
% + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{v,n}^C\}\right]}_{\textbf{Part C, Variance event does not hold}} \\
%%%%%%%%%%%%%%
% &\qquad + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{s,n}^C\}\right]}_{\textbf{Part D, Safety event does not hold}} 
&\quad + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi^C_{c,n}}\right]}_{\textbf{Part C, Safety event does not hold}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right]}{\underline{T}^2_{n}(a)} + \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi^C_{Z,n}\}\right]}{\underline{T}^2_{n}(a)} + \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi^C_{c,n}\}\right]}{\underline{T}^2_{n}(a)}
\end{align*}
Divide the total budget $n$ into two parts, $n_{f}$ when $\sum_{\ell=1}^n\indic{\wZ_t \geq 0}$ is true, then any action from $\{0\}\bigcup\A$ can be sampled. Hence,
$\sum_{a=0}^A\E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right]=n_{f}$. 
The other part consist of $n_{u} = n-n_{f}$ samples when $\sum_{\ell=1}^n\indic{\wZ_\ell < 0}$ and only action $\{0\}$ is sampled. Hence,
$\E\left[T_{n}(0)\mathbb{I}\{\xi_{c,n}\cap\xi^C_{Z,n}\}\right]=n_{f}$. 
% We further divide the number of actions allocated to safe actions in $\sA$ when $\sum_{\ell=1}^n\indic{\wZ_t \geq 0}$ as $n_{safe, \sA}$ and to unsafe actions as $n_{safe, \uA}$. 

\textbf{Step 3 (Sampling of oracle for $\wZ_\ell \geq 0$):} First note that when $\wZ_\ell\geq 0$ the oracle samples at round $\ell$ the action $\argmax_a U_{\ell+1}(a)$ where
\begin{align}
U_{\ell+1}(a') &\coloneqq\frac{\pi(a')}{T_{\ell}(a')}\sigma(a') \label{eq:oracle-1}
%%%%%%%%%%%%%%%
\end{align}
Let $\ell+1>2 K$ be the time at which a given action $k$ is pulled for the last time, i.e., $T_{\ell}(k)=T_{n}(k)-1$ and $T_{\ell+1}(k)=T_{n}(k)$. This is because $T_{n_f}(a) = T_n(a)$ for $a\in\A\setminus\{0\}$ as for $n_u$ samples oracle selects only action $0$. Note that as $n \geq 4 A$, there is at least one action $p'$ such that this happens, i.e. such that it is pulled after the initialization phase. Since the oracle chooses to pull action $p'$ at time $\ell+1$, we have for any action $p$
\begin{align}
U_{\ell+1}(p) \leq U_{\ell+1}(p') .\label{eq:oracle-2}
\end{align}
From \eqref{eq:oracle-1} and using the fact that $T_{\ell}(p')=T_{n}(p')-1$, we can show that
\begin{align}
U_{\ell+1}(k) \leq \frac{\pi(p')}{T_{\ell}(k)}\sigma(k)=\frac{\pi(p')}{T_{n}(p')-1}\sigma(p') \label{eq:oracle-3}
\end{align}
Also, note that
\begin{align}
    U_{\ell+1}(p) = \frac{\pi(p)}{T_{\ell}(p)}\sigma(p) \overset{(a)}{\geq} \frac{\pi(p)}{T_{n}(p)}\sigma(p). \label{eq:oracle-4}
\end{align}
where, $(a)$ follows as $T_{\ell}(p)\leq T_{n}(p)$ (i.e., the number of times $p$ has been pulled can only increase after time $\ell$). 
Combining \eqref{eq:oracle-2}, \eqref{eq:oracle-3}, \eqref{eq:oracle-4} we can show that for any action $p$:
\begin{align}
    \frac{\pi(p)}{T_{n}(p)}\sigma(p) \leq \frac{\pi(k)}{T_{n}(p')-1}\sigma(p') \label{eq:oracle-5}
\end{align}
Note that in the above equation, there is no dependency on $\ell$, and thus, the probability that \eqref{eq:oracle-5} holds for any $p$ and for any $k$ such that action $k$ is pulled after the initialization phase, i.e., such that $T_{n}(k)>2$ depends on the probability of event $\xi_{Z,n}$.

\textbf{Step 4. (Lower bound on $T_{n}(p)$ for $\wZ_t \geq 0$):} If an action $p$ is under-pulled compared to its optimal allocation without taking into account the initialization phase, i.e., $T_{n}(p)-2<\bb(p)(n-2 A)$, then from the constraint $\sum_{p'}\left(T_{n}(p')-2\right)=n-2 A$ and the definition of the optimal allocation, we deduce that there exists at least another action $p'$ that is over-pulled compared to its optimal allocation without taking into account the initialization phase, i.e., $T_{n}(p')-2>\bb(p')(n-2 A)$. Note that for this action, $T_{n}(p')-2>\bb(p')(n-2 A) \geq 0$, so we know that this specific action is pulled at least once after the initialization phase and that it satisfies \eqref{eq:oracle-5}. 
Recall that we have defined $M = \sum_a \pi(a)\sigma(a)$. Using the definition of the optimal allocation $T_{n}(p')^*=n_f \frac{\pi(p') \sigma(p')}{M}$, and the fact that $T_{n}(p') \geq \bb(k)(n_f-$ $2 A)+2$, \eqref{eq:oracle-5} may be written as for any action $p$
\begin{align}
\frac{\pi(p) \sigma(p)}{T_{n}(p)} & \leq \frac{\pi(p')}{T_{n}(p')^*} \frac{n_f}{(n_f-2 A)}\sigma(p') \leq \dfrac{M}{n_f} + \dfrac{4 A M}{n_f^2} \label{eq:oracle-6}
\end{align}
because $n_f \geq 4 A$. 
By rearranging \eqref{eq:oracle-6}, we obtain the lower bound on $T_{n}(p)$ :
\begin{align}
T_{n}(p) \geq \frac{\pi(p) \sigma(p)}{\frac{M}{n_f}+\frac{4 A M}{n_f^2}} = \dfrac{\pi(p) \sigma(p)}{\frac{M}{n_f}\left(1 + \frac{4A}{n_f}\right)} \overset{(a)}{\geq} T^*_{n}(p)-4 A \bb^*(p), \label{eq:oracle-6-1}
\end{align}
where in $(a)$ we use $1 /(1+x) \geq 1-x$ (for $x>-1$ ). Note that the lower bound holds on $\xi_{c,n}$ for any action $p$.


\textbf{Step 5. (Upper bound on $T_{n}(p)$ for $\wZ_\ell \geq 0$):} Now using \eqref{eq:oracle-6-1} and the fact that $\sum_a T_{n}(a)=n_f$, we obtain
\begin{align*}
T_{n}(p)=n_f-\sum_{k \neq p} T_{n}(k) \leq\left(n_f -\sum_{p' \neq p} T_{n}^*(p')\right)+\sum_{p' \neq p}4 A \bb^*(k) .
\end{align*}
Now since $\sum_{p' \neq p} \bb^*(p') \leq 1$ we can show that
\begin{align}
T_{n}(p) \leq T_{n}^*(p)+4 A . \label{eq:oracle-6-2}
\end{align}



\textbf{Step 6 (Bound part A):} We now bound the part A using \eqref{eq:oracle-6}
\begin{align*}
    % \sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right] &\leq
    % %%%%
    \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right]}{\underline{T}^2_{n}(a)}%\\
    %%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq} \left(\frac{M }{n_f}+\frac{4 A M}{n_f^2}\right)^2 n_{f} %\\
    %%%%%%%%%%%%%
    \overset{}{=} \frac{M^2}{n_f}+\frac{8A M^2}{n_f^2} + \frac{16A^2 M^2}{n_f^3}
\end{align*}
where, in $(a)$ we have that $M = \sum_a \pi(a)\sigma(a)$ and $\sum_a\E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right]=n_{f}$.
% , $(b)$ follows as $n_{f}\leq n$.


\textbf{Step 7 (Upper bound bound to Constraint violation):} In this step we bound the quantity $\C^*_n(\pi) = \sum_{\ell=1}^n\indic{\wZ_\ell < 0, A_t\sim \{\bb^*, \pi_0\}}$. Observe that $\C^*_n(\pi) = \sum_{\ell=1}^n\indic{\wZ_t < 0, A_t\sim \{\bb^*, \pi_0\}} = T_n(0)\indic{\xi^C_{Z,n}}$ as when the constraint are violated action $\{0\}$ is sampled. 
Let $\tau=\min \left\{\ell \leq n \text{ and } n_f \geq \frac{\log(An(n+1)/\delta)}{\min_{a\in\A\setminus\{0\}}\pi(a)\sigma(a)\Delta^{c,\alpha,(2)}(a)} \mid I_\ell=0\right\}$ be the last round in which the baseline action is played. We will define formally the gap $\Delta^{c,\alpha,(2)}(a)$ later. Since $\xi_{c,n}$ holds and
\begin{align*}
    \wmu^c_\ell(0) + C_\ell(0) < \max_a\wmu^c_\ell(a) < \max_a\wmu^c_\ell(a) + C_\ell(a).
\end{align*}
Note that we can sample the default action $0$ for two reasons. If the safety budget $\wZ_\ell \geq 0$ and
$$
\dfrac{\pi(0)\sigma(0)}{T_\ell(0)} > \dfrac{\pi(a)\sigma(a)}{T_\ell(a)}
$$ 
for all $a\in\A\setminus\{0\}$.  
This is handled in steps 3 and 4. Now in this step we focus on when $\wZ_\ell < 0$. Note that in this case we only sample action $0$ if $\wZ_\ell(0) < 0$. Let $J_\ell = \argmax_a\frac{\pi(a)\sigma(a) }{T_\ell(a)}$. Define the LCB for an action $a$ as $\underline{\wmu}^c_\ell(a) = \mu^c(a) - C_\ell(a)$. It follows then
\begin{align}
\sum_{a=0}^A T_{\tau-1}(a) \underline{\wmu}^c_{\tau}(a)+\underline{\wmu}^c_{\tau}(J_\tau)-(1-\alpha) \mu^c(0) \tau<0 \label{eq:oracle-7}
\end{align}
By dropping $\underline{\wmu}_{\tau}(J_\tau)$, replacing $\tau$ in \eqref{eq:oracle-7} with $\sum_{a=0}^A T_{\tau-1}(a)+1$, and rearranging the terms in \Cref{eq:oracle-7}, we get
\begin{align}
\alpha T_{\tau-1}(0) \mu^c(0) &<(1-\alpha) \mu^c(0)+\sum_{a=1}^A T_{\tau-1}(a)\left((1-\alpha) \mu^c(0)-\underline{\wmu}^c_{\tau}(a)\right) \nonumber\\
%%%%%%%%%%%%
& \leq(1-\alpha) \mu^c(0) 
+\sum_{a=1}^A T_{\tau-1}(a)\left((1-\alpha) \mu^c(0)-\mu^c(a)+c_1\sqrt{\frac{\log(An(n+1)/\delta)}{T_{\tau-1}(a)}}\right) \nonumber\\
%%%%%%%%%%%%
& \leq 1+\sum_{a=1}^A N(a) \implies T_{\tau-1}(0) \leq \dfrac{1}{\alpha\mu^c(0)}\left(1+\sum_{a=1}^A N(a)\right) . \label{eq:oracle-8}
\end{align}
where $\Delta^{c,\alpha}(a)\coloneqq(1-\alpha) \mu^c(0)-\mu^c(a)$ and
\begin{align*}
N(a) &\coloneqq T_{\tau-1}(a) \cdot\left((1-\alpha) \mu^c(0)-\mu^c(a)+c_1\sqrt{\log(An(n+1)/\delta) / T_{\tau-1}(a)}\right) \\
&=\Delta^{c,\alpha}(a) T_{\tau-1}(a)+c_1\sqrt{\log(An(n+1)/\delta) T_{\tau-1}(a)}
\end{align*}
is a bound on the decrease in $\wZ_\tau$ in the first $\tau-1$ rounds due to choosing action $a$. We will now bound $N(a)$ for each $a>0$. Now observe
\begin{align*}
    \Delta^{c,\alpha}(a) = (1-\alpha) \mu^c(0)-\mu^c(a) = \mu^c(0) - \alpha\mu^c(0) - \mu^c(a) &= -(\mu^{*,c} - \mu^c(0)) - \alpha\mu^c(0) + (\mu^{*,c} - \mu^c(a)) \\
    %%%%%%%%%%%%%%%%%%
    &= -\Delta^c(0) - \alpha\mu^c(0) + \Delta^c(a).
\end{align*}
where, $\mu^{*,c} = \max_a\mu^c(a)$. The first case is $\Delta^{c,\alpha}(a) > 0$, i.e. $\Delta^c(a) > \Delta^c(0)+\alpha \mu^c(0)$. These are the unsafe actions as $\Delta^{c,\alpha}(a) \coloneqq(1-\alpha) \mu^c(0)-\mu^c(a) > 0$ we have from \eqref{eq:oracle-6-2}
\begin{align*}
    T_n(a) &\leq T^*_n(a) + 4A
    %%%%%%%%%%%%
    = \dfrac{\pi(a)\sigma(a)}{M}n_f +  4A
\end{align*}
Plugging this back in $N(a)$ we get
\begin{align}
    N(a) &=\Delta^{c,\alpha}(a) T_{\tau-1}(a)+c_1\sqrt{\log(An(n+1)/\delta) T_{\tau-1}(a)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%
    &\leq \dfrac{\pi(a)\sigma(a)}{M}n_f\Delta^{c,\alpha}(a) + 4A\Delta^{c,\alpha}(a) + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%%
    % &= \dfrac{\pi(a)\sigma(a)}{M}n_f\Delta^{c,\alpha}(a) + 4A\Delta^{c,\alpha}(a) + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}(n - n_u) + 4A\right)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq} \dfrac{\pi(a)\sigma(a)}{M}n_f\Delta^{c,\alpha}(a) + 4A\Delta^{c,\alpha}(a) + c_1\sqrt{\Delta^{c,\alpha,(2)}(a)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%%
    % c_1\sqrt{\log(An(n+1)/\delta)}
    &\overset{}{\leq} 2\left(\dfrac{\pi(a)\sigma(a)}{M}n_f\Delta^{c,\alpha}(a) + 4A\Delta^{c,\alpha}(a)\right) 
    % \nonumber\\
    % + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%%%
    % &\overset{(a)}{\leq} \dfrac{1}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right) + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right)} 
    \label{eq:oracle-9} 
\end{align}
where, $(a)$ follows for $n_f \geq \frac{\log(An(n+1)/\delta)}{\min_a\Delta^{c,\alpha,(2)}(a)}$.
% $\dfrac{\log(An(n+1)/\delta)}{n} \leq 4 \left(\sum_{\A\setminus\{0\}}\pi(a)\sigma(a)\max{\Delta^c(a),\Delta^c(0)-\Delta^C(a)}\right)^2$.
%
% as $\Delta^{c,\alpha}(a)$.
% \begin{align*}
%     &\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right)} \leq \Delta^{c,\alpha}(a)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 4A\right) \\
%     %%%%%%%%%%%%%%%%%%%%%%
%     \implies \log(An(n+1)/\delta) &\leq \Delta^{c,\alpha,(2)}(a)
% \end{align*}
%
%
The other case is $\Delta^{c,\alpha}(a)< 0$, i.e. $\Delta^c(a)<\Delta^c(0)+\alpha \mu^c(0)$ then only safe actions are pulled. Then
\begin{align}
N(a) &\leq -\Delta^{c,\alpha}(a)T_{\tau-1}(a) + c_1\sqrt{\log(An(n+1)/\delta) T_{\tau-1}(a)} = \underbrace{-\Delta^{c,\alpha}(a)}_{a}T_{\tau-1}(a) + \underbrace{c_1\sqrt{\log(An(n+1)/\delta)}}_{b}\sqrt{T_{\tau-1}(a)}\nonumber\\
%%%%%%%%%%%%%%%%%%
&\overset{(a)}{\leq} -\dfrac{\log(An(n+1)/\delta)}{4\Delta^{c,\alpha}(a)} = \dfrac{\log(An(n+1)/\delta)}{4(\Delta^c(0) + \alpha\mu^c(0) - \Delta^c(a))} \overset{(b)}{\leq} 4 \left(\dfrac{\pi(a)\sigma(a)}{M}n_f(\Delta^c(0) + \alpha\mu^c(0) - \Delta^c(a)) \right) 
%%%%%%%%%%%%%%%%%%%
\label{eq:oracle-10}
\end{align}
where, $(a)$ follows by using $a x^2+b x \leq-b^2 / 4 a$ for $a<0$, and $(b)$ follows as $n_f \geq \frac{\log(An(n+1)/\delta)}{\min^{+}_{a\in\A\setminus\{0\}}\pi(a)\sigma(a)\Delta^{c,\alpha,(2)}(a)}$ which implies
\begin{align*}
&\dfrac{\log(An(n+1)/\delta)}{n_f} \leq 4 \left(\sum_{\A\setminus\{0\}}\pi(a)\sigma(a)\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a)\}\right)^2 \\
%%%%%%%%%%%%%%%%%%%
&\implies \dfrac{\log(An(n+1)/\delta)}{\sum_{\A\setminus\{0\}}\pi(a)\sigma(a)\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a)\}} \leq 4 \left(\sum_{\A\setminus\{0\}}\pi(a)\sigma(a)\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a)\}\right)n_f
\end{align*}
%
%
%
% From \eqref{eq:oracle-9} 
% for $a\in\uA$, the set of unsafe actions, gives
% \begin{align*}
% N(a) &\leq \dfrac{1}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 8A\right) + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f + 8A\right)}\\
% %%%%%%%%%%%%%%%%%%
% &\overset{(a)}{\leq} \dfrac{1}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n_f\right) + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f \right)}\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &\overset{(b)}{\leq} \dfrac{1}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M }n_f \right) + \log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M }n_f \right)\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &\overset{(c)}{\leq} \dfrac{2\log(An(n+1)/\delta)}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M }n_f\right) 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% \end{align*}
% where, $(a)$ follows as $A\leq \sqrt{n_f}$ so we can subsume the $8A$ into the leading term $c_1\sqrt{n\log(An(n+1)/\delta)}$, 
% $(b)$ follows as 
% \begin{align*}
%     \left(\dfrac{\pi(a)\sigma(a)}{M }n_f\right) \geq \sqrt{\left(\dfrac{\pi(a)\sigma(a)}{M }n_f \right)}.
% \end{align*}
% The $(c)$ follows as $\min^{+}\{\log(An(n+1)/\delta),\Delta^{c,\alpha}(a)\}\leq 2\log(An(n+1)/\delta)/\Delta^{c,\alpha}(a)$. Similarly for $a\in\sA$, the set of safe actions we can show that
% \begin{align*}
%     N(a) \leq \dfrac{\log(An(n+1)/\delta)}{4(\Delta^c(0) + \alpha\mu^c(0) - \Delta^c(a))} \overset{(a)}{\leq} \dfrac{2\log(An(n+1)/\delta)}{4(\Delta^c(0) + \alpha\mu^c(0) - \Delta^c(a))}\left(\dfrac{\pi(a)\sigma(a)}{M}n_f \right)
% \end{align*}
% where, $(a)$ follows by inserting $\left(\frac{\pi(a)\sigma(a)}{M}n_f \right) >1$ for the quantity $\frac{2\log(An(n+1)/\delta)}{4(\Delta^c(0) + \alpha\mu^c(0) - \Delta^c(a))}$. Observe that this term consists of the safe action, so we insert $\left(\frac{\pi(a)\sigma(a)}{M}n_f\right)$. 
%
%
%
Plugging everything back in \eqref{eq:oracle-10}, we get
\begin{align}
n_u &=T_{\tau-1}(0) = \dfrac{1}{\alpha\mu^c(0)}\left(\sum_{a=1}^A N(a)\right)\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq 
% \frac{2 A+2}{\alpha \mu^c(0)}+
\frac{2}{\alpha \mu^c(0)} \sum_{a\in\uA}
\Delta^c(a)
\left(\dfrac{\pi(a)\sigma(a)}{M}n_f \right) 
%%%%%%
+ \frac{4}{\alpha \mu^c(0)}\sum_{a\in\sA\setminus\{0\}}\left(\Delta^c(0)-\Delta^c(a) \right)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f \right)\nonumber\\
%%%%%%%%%%%%%%%%%%
&= 
% \frac{2 A+2}{\alpha \mu^c(0)}+
\frac{6}{\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\left(\dfrac{\pi(a)\sigma(a)}{M}(n - n_u) \right)
% \nonumber\\
%%%%%%%%%%%%%%%%%%
% &= 
% \frac{2 A+2}{\alpha \mu^c(0)}+ 
% \dfrac{6H_*}{1+6H_*}\dfrac{n}{M} 
\overset{}{\leq} \dfrac{H_*}{2}\dfrac{n}{M}.
% \nonumber\\
%%%%%%%%%%%%%%%%%%
% &= \frac{2 A+2}{\alpha \mu^c(0)H_*} + 
\label{eq:oracle-11}
\end{align}
% where, $(a)$ follows for $H_* \leq \frac{1}{2}$. 

% \begin{align*}
%     n_u &= C + \sqrt{\log n} H_*(n-n_u)\\
%     %%%%%%%%%%
%     n_u(1 + \sqrt{\log n} H_*)&=  C + n\sqrt{\log n} H_*\\
%     n_u &= \dfrac{C + n\sqrt{\log n} H_*}{1 + \sqrt{\log n} H_*} = \dfrac{C}{1 + b} + (b/1+b) n
% \end{align*}


% Observe, that for safe action small $\Delta^c(0) - \Delta^c(a)$ implies that action $a$ is close to the $\mu^c(0)$. This implies that safe action close to the $\mu^c(0)$ is allocated more samples.

\textbf{Step 8 (Lower bound to Constraint violation):} To bound the lower bound of $T_n(0)$ for $\wZ_\ell < 0$ we equate the safety budget to $0$. It follows then
\begin{align}
\sum_{a=0}^A T_{\tau-1}(a) \underline{\wmu}^c_{\tau}(a)+\underline{\wmu}^c_{\tau}(J_\tau)-(1-\alpha) \mu^c(0) \tau = 0 \label{eq:oracle-7-1}
\end{align}
By dropping $\underline{\wmu}^c_{\tau}(J_\tau)$, replacing $\tau$ in \eqref{eq:oracle-7-1} with $\sum_{a=0}^A T_{\tau-1}(a)+1$, and rearranging the terms in \Cref{eq:oracle-7-1}, we get
\begin{align}
\alpha T_{\tau-1}(0) \mu^c(0) & > (1-\alpha) \mu^c(0)+\sum_{a=1}^A T_{\tau-1}(a)\left((1-\alpha) \mu^c(0)-G_{\tau}(a)\right) \nonumber\\
%%%%%%%%%%%%
& =(1-\alpha) \mu^c(0) 
+\sum_{a=1}^A T_{\tau-1}(a)\left((1-\alpha) \mu^c(0)-\mu^c(a) + c_1\sqrt{\frac{\log(An(n+1)/\delta)}{T_{\tau-1}(a)}}\right) \nonumber\\
%%%%%%%%%%%%
& = 1+\sum_{a=1}^A \underline{N}(a) \implies T_{\tau-1}(0) \geq \dfrac{1}{\alpha\mu^c(0)}\left(1 +\sum_{a=1}^A \underline{N}(a)\right) . \label{eq:oracle-8-1}
\end{align}


These are the unsafe actions (see the definition of $\Delta^{c,\alpha}(a))$ we have from \eqref{eq:oracle-6-2}
\begin{align*}
    T_n(a) &\geq T^*_n(a) - 4A\bb^*(a)
    %%%%%%%%%%%%
    = \dfrac{\pi(a)\sigma(a)}{M}n_f  - 4A\bb^*(a)
\end{align*}
Plugging this back in $N(a)$ we get
\begin{align}
    \underline{N}(a) &=\Delta^{c,\alpha}(a) T_{\tau-1}(a)+c_1\sqrt{\log(An(n+1)/\delta) T_{\tau-1}(a)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%
    &\geq \dfrac{\pi(a)\sigma(a)}{M}n_f\Delta^{c,\alpha}(a) - 4\bb(a)A\Delta^{c,\alpha}(a) + c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - 4\bb^*(a)A\right)} \nonumber\\
    %%%%%%%%%%%%%%%%%%%%%
    &\geq \dfrac{\pi(a)\sigma(a)}{M}n_f\Delta^{c,\alpha}(a) - 4\bb^*(a)A\Delta^{c,\alpha}(a) 
    \label{eq:oracle-9-1} 
\end{align}
%
%
%
% where, $(a)$ follows as for $\sqrt{n}\geq \dfrac{Mc_1\sqrt{A}\log(An(n+1)/\delta)}{\pi_{\min^{+}}\sigma_{\min^{+}}} + 4A$ we can show the following
% \begin{align*}
%     &\Delta^{c,\alpha}(a)\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4\bb(a)A\right) - c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4\bb(a)A\right)} \geq \dfrac{1}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4A\bb(a)\right)\\
%     %%%%%%%%%%%%%%%%%%%%%%%%%
%     \implies & \left(\Delta^{c,\alpha}(a) - \dfrac{1}{\Delta^{c,\alpha}(a)}\right)\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4\bb(a)A\right)\geq c_1\sqrt{\log(An(n+1)/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4\bb(a)A\right)}\\
%     %%%%%%%%%%%%%%%%%%%%%%%
%     \overset{(a)}{\implies} & \left(\Delta^{c,\alpha}(a) - \dfrac{1}{\Delta^{c,\alpha}(a)}\right)^2\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4\bb(a)A\right)\geq \log(An(n+1)/\delta)\\
%     %%%%%%%%%%%%%%%%%%%%%%
%     \implies & n \geq \dfrac{M}{\pi(a)\sigma(a)}\dfrac{\log(An(n+1)/\delta)}{\left(\Delta^{c,\alpha}(a) - \dfrac{1}{\Delta^{c,\alpha}(a)}\right)^2} + 4A\\
%     %%%%%%%%%%%%%%%%%%
%     \implies & n \geq \dfrac{M}{\pi(a)\sigma(a)}\dfrac{\log(An(n+1)/\delta)}{\left(\dfrac{n-A}{\sqrt{An}}\right)^2} + 4A\\
%     %%%%%%%%%%%%%%%%%%%
%     \implies & \sqrt{n} \geq \dfrac{M\sqrt{A}\log(An(n+1)/\delta)}{\pi(a)\sigma(a)} + 4A
% \end{align*}
% where $(a)$ follows by squaring both sides and noting that $\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4\bb(a)A\right) > 0$. 
%
%
%
The other case is $\Delta^{c,\alpha}(a)< 0$, i.e. $\Delta(a)<\Delta(0)+\alpha \mu^c(0)$ then only safe actions are pulled. Then
\begin{align}
\underline{N}(a) &= -\Delta^{c,\alpha}(a)T_{\tau-1}(a) + c_1\sqrt{\log(An(n+1)/\delta) T_{\tau-1}(a)} \leq \underbrace{(1-\Delta^{c,\alpha}(a))}_{a}T_{\tau-1}(a) + \underbrace{c_1\sqrt{\log(An(n+1)/\delta)}}_{b}\sqrt{T_{\tau-1}(a)}\nonumber%\\
\end{align}
This implies that $\underline{N}(a)$ has a minimum  given by $\underline{N}(a) \geq b^2/2a$. It follows then that
\begin{align}
%%%%%%%%%%%%%%%%%%
&\underline{N}(a)\overset{(a)}{\geq} \dfrac{\log(An(n+1)/\delta)}{4(1-\Delta^{c,\alpha}(a))} \overset{(b)}{\geq} \dfrac{\log(An(n+1)/\delta)}{8\Delta^{c,\alpha}(a)} = \dfrac{\log(An(n+1)/\delta)}{8(\Delta(0) + \alpha\mu^c(0) - \Delta(a))}\overset{(c)}{\geq} \frac{1}{8} \left(\dfrac{\pi(a)\sigma(a)}{M}n_f(\Delta^c(0) + \alpha\mu^c(0) - \Delta^c(a)) \right) 
%%%%%%%%%%%%%%%%%%%
\label{eq:oracle-10-1}
\end{align}
where, $(a)$ follows by using $a x^2+b x \geq b^2 / 4 a$ for $a>0$, $(b)$ follows as $\Delta^\alpha(a) < 0$, and $(c)$ follows for $\frac{\log(An(n+1)/\delta)}{n_f} \leq 4 \left(\sum_{\A\setminus\{0\}}\pi(a)\sigma(a)\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^C(a)\}\right)^2$.  
%
%
% Continuing from \eqref{eq:oracle-9-1} 
% % to \eqref{eq:oracle-10} 
% for $a\in\uA$ gives
% \begin{align*}
% N(a) &\geq \dfrac{1}{\Delta^{c,\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n - 4A\bb(a)\right) 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% \end{align*}
%
%
Plugging everything back in \eqref{eq:oracle-8-1}, we get
\begin{align}
&T_{\tau-1}(0) \geq  \dfrac{1}{\alpha\mu^c(0)}\left(1 + \sum_{a=1}^A N(a)\right)\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(a)}{\geq} 1 +  \frac{1}{\alpha \mu^c(0)} \sum_{a\in\uA}\Delta^c(a)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - 4A\bb^*(a)\right) +
 \frac{1}{\alpha \mu^c(0)}\sum_{a\in\sA\setminus\{0\}}(\Delta^c(0)-\Delta^c(a) )\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - 4A\bb^*(a)\right) 
\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%
&\geq 1 + \frac{1}{8\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - 4A\bb^*(a)\right) \nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(b)}{=} \dfrac{H_*}{8}\dfrac{n_f}{M} - \frac{A}{2\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\bb^*(a)
\nonumber\\
%%%%%%%%%%%%%%%%%%%%
&\overset{}{=} \dfrac{n_f}{M}\left(\dfrac{H_*}{8} - \dfrac{M}{n_f}\left(\frac{A}{2\alpha \mu^c(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\bb^*(a)\right) \right)\label{eq:oracle-11-1}
\end{align}
where, $(a)$ follows as $\alpha \mu^c(0) \geq 1$, $(b)$ follows from the definition of $H_*$.
% and $(c)$ follows from $\bb^*(a) = \frac{\pi(a)\sigma(a)}{M}n_f$
%
% Observe, that for safe action small $\Delta^c(0) - \Delta^c(a)$ implies that action $a$ is close to the $\mu^c(0)$. This implies that safe action close to the $\mu^c(0)$ is allocated more samples.
%
Observe that from
%from \eqref{eq:oracle-6-1} and 
\eqref{eq:oracle-11-1} we have that
\begin{align}
    T_n(0) &\overset{(a)}{\geq} \dfrac{n_f}{M}\left(\dfrac{H_*}{8}  - \dfrac{M}{n_f}\left(\frac{A}{2\alpha \mu^c(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\dfrac{\pi(a)\sigma(a) n_f}{M}\right) \right)\nonumber\\
    %%%%%%%%%%%%%%%
    &= \dfrac{n_f}{M}\left(\dfrac{H_*}{8} - \frac{A}{2}\dfrac{H_*}{M}  \right). \label{eq:bandit-constraint-lower-bound}
    % \overset{(a)}{\geq} \left(1 - \dfrac{A}{4M} + \dfrac{H_*}{8}\right)\dfrac{n_f}{M}
\end{align}
where, $(a)$ follows for $\bb^*(a) = \frac{\pi(a)\sigma(a)}{M}n_f$.
 
%\frac{1}{8\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\left(\pi(a)\sigma(a) - 4A\bb(a)\dfrac{M}{n_f}\right)
\textbf{Step 9 (Bound Part B)}: Then from \eqref{eq:oracle-11-1} we can show that
\begin{align*}
   \dfrac{\pi(0)\sigma(0)}{T_n(0)} \leq \dfrac{M }{n_f}\dfrac{\pi(0)\sigma(0)}{  \dfrac{H_*}{8} - \dfrac{A H_*}{2M}  }%\\
   %%%%%%%%%%%%%%%%%
   &\overset{}{\leq} \dfrac{M \pi(0)\sigma(0)}{n_f}\left(2 + \dfrac{H_*}{8} + \dfrac{A H_*}{2M}\right)\overset{(a)}{\leq} \dfrac{M A \pi(0)\sigma(0)}{n_f}\left(2 + H_*\right) %\\
   %%%%%%%%%%%%%%%%
   % &\dfrac{M \pi(0)\sigma(0)}{n_f}(2 + H_*)
\end{align*}
where, $(a)$ follows for $A\geq 2$.
% $1/1+m \leq 2 + m$ for $ m\geq 0$. 
It follows then by setting $\E\left[T_{n}(0)\indic{\xi^C_{Z,n}}\right]\leq n_u$ and setting $n_f = n - n_u$ that 
\begin{align*}
    \frac{\pi(0)^2 \sigma(0)^2 \E\left[T_{n}(0)\indic{\xi_{Z,n}}^C\right]}{\underline{T}^2_{n}(0)} 
    % \leq \dfrac{M^2 \pi^2(0)\sigma^2(0)}{n_f^2}\left(2 + \frac{1}{\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\pi(a)\sigma(a)\right)^2 n_u\\
    %%%%%%%%%%%%%%%%%%%%
    % &\leq \dfrac{M^2 \pi^2(0)\sigma^2(0) n_u}{(n-n_u)^2}\bigg(4 + \dfrac{4}{\alpha \mu^c(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\pi(a)\sigma(a) \\
    %%
    % &\quad + \frac{1}{\alpha^2 \mu^{c,(2)}(0)}\left(\sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\pi(a)\sigma(a)\right)^2\bigg)\\
    %%%%%%%%%%%%%%%%%%%%%%
    & = \dfrac{M^2 A^2 \pi^2(0)\sigma^2(0) n_u}{(n-n_u)^2}\left(2 + H_*\right)^2\\
    % \left(4 + \dfrac{4 H_*}{\pi(0)\sigma(0)} + \frac{H^2_*}{\pi^2(0)\sigma^2(0)}\right) \\
    %%%%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq } \dfrac{M^2 A^2 \pi^2(0)\sigma^2(0) H_* n}{(n-H_*n)^2}\left(2 + H_*\right)^2 \\
    %%%%%%%%%%%%%%%%%%%%
    &\leq \dfrac{M^2 A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2
\end{align*}
where, $(a)$ follows from \eqref{eq:oracle-11}.
% the $H_*$ is a problem-dependent parameter defined as 
% \begin{align*}
%     H_* = \dfrac{1}{\alpha\mu^c(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\pi(a)\sigma(a)
% \end{align*}






\textbf{Step 10 (Combine everything):} Combining everything from step 5, step 8 and setting $\delta=1/n^2$ we can show that the MSE of oracle scales as
\begin{align}
    \L_n(\pi) &\leq \frac{M^2}{n_f}+\frac{8A M^2}{n_f^2} + \frac{16A^2 M^2}{n_f^3} + \dfrac{M^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 %\\
    %%%%%%%%%%%%%%%%%%%
    + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu^c_{n}(a)-\mu^c(a)\right)^2\indic{\xi_{c,n}}^C\right]}_{\textbf{Part C, Safety event does not hold}}\nonumber\\
    %%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq} \frac{M^2}{n - n_u}+\frac{16A M^2}{(n - n_u)^2} + \frac{16A^2 M^2}{(n - n_u)^3} + \dfrac{M^2A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + 2\sum_{\ell=1}^n\dfrac{2\eta + 4\eta^2}{n^2}\nonumber\\
    %%%%%%%%%%%%%%%%%%%
    &\overset{(b)}{\leq} \frac{M^2}{n - H_* n/2 M}+\frac{16A M^2}{(n - H_* n/2 M)^2} + \frac{16A^2 M^2}{(n - H_* n/2 M)^3} + \dfrac{M^2A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + \dfrac{2}{n}\nonumber\\
    %%%%%%%%%%%%%%%%%%
    % &\overset{(c)}{\leq} \frac{M^3}{n(2M - H_*) }+\frac{16A M^4}{n^2(2M - H_*)^2} + \frac{16A^2 M^5}{n^3(2M - H_*)^3} + \dfrac{M^2A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + \dfrac{2}{n} \\
    %%%%%%%%%%%%%%%%%%%%
    &\overset{(c)}{\leq} \frac{M^2}{n}+\frac{16A M^2}{n^2} + \frac{16A^2 M^2}{n^3} + \dfrac{M^2A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + \dfrac{2}{n}
    \label{eq:bandit-final-loss-oracle}
\end{align}
where, $(a)$ follows as $\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu^c_{n}(a)-\mu^c(a)\right)^2\right] \leq 2\eta + 4\eta^2$ and using the low error probability of the cost event from \Cref{lemma:conc-mu}. The $(b)$ follows by substituting $n_u \leq \frac{H_*}{2}\frac{n}{M}$, and $(c)$ follows by considering the leading terms. 
The claim of the theorem follows.
\end{proof}


\begin{remark}
\label{rem:pi-e}
\textbf{(Exploration policy $\pi_e$):}
The exploratory policy $\pi_e$ samples each action in each state $\frac{\log(SAn(n+1)/\delta) }{\min_{s,a}\Delta^{c,(2)}(s,a)}$ number of times. This is a deterministic action selection rule. We can show from \Cref{corollary:safe-conc} that this result in a good cost estimate for each state-action tuple $(s,a)$. Define the following event
\begin{align*}
    \overline{\xi}_{\delta} = \bigcap_{s\in\S}\bigcap_{1 \leq a \leq A, T_n(s,a) \geq 1}\left\{\left|\frac{1}{T_n(s,a)}\sum_{t=1}^{T_n(s,a)} C_{t}(s, a)-\mu^c(s, a)\right| \geq (2\eta + 4\eta^2) \sqrt{\frac{\log (SA n(n+1) / \delta)}{2 T_n(s,a)}}\right\}. 
\end{align*}
It then follows from \Cref{corollary:safe-conc} that $\Pb(\overline{\xi}_{\delta}) \leq \delta$. For this event to hold true with high probability, the $\pi_e$ requires an exploration budget of greater than $\frac{SA \log(SAn(n+1)/\delta) }{\min_{s,a}\Delta^{c,(2)}(s,a)}$.
\end{remark}









==> saver_regret.tex <==
\begin{customtheorem}{2}\textbf{(formal)}
    The MSE of the oracle for $\frac{n}{\log(An(n+1)/\delta)} \geq 4A + \frac{A}{\min_{a}\Delta^{c,(2)}(a)} + \frac{1}{4 H_*^2}$ is bounded by
    \begin{align*}
        % \L_n(\pi) \leq \frac{M^2}{n}+\frac{16A M^2}{n^2} + \frac{16A^2 M^3}{n^3} + \dfrac{M^2A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + \dfrac{2}{n}
        \L_n(\pi) \leq &\frac{M^2}{n}+\frac{8A M^2}{n^2} + \frac{16A^2 M^3}{n^3} + 2M^{5/2} \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{3/2}} \nonumber\\ 
        %%%%%%%%%
        &\qquad + 8AM^{5/2}\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{3/2}} + \dfrac{M^2(2\eta + 4\eta^2)^2\log (A n(n+1) / \delta)}{\bb^{*,3}_{\min} n^2}\nonumber\\
        %%%%%%%%%%
        &\qquad + \dfrac{M^2 A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 5/2}_{\min}n^{5/2}}\right) + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 3/2}_{\min}n^{3/2}}\right)
        %%%%%%%%%%%%%%%%
        + \dfrac{2}{n}
    \end{align*}
    with probability $(1-\delta)$. The $H_* = \frac{1}{\alpha\mu(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta(a),\Delta(0)-\Delta(a) \}\pi(a)\sigma(a)$ is the problem complexity parameter. The total predicted constraint violations is bounded by
    \begin{align*}
        \C_n(\pi) \leq \dfrac{H_* n}{2 M}
        % \frac{1}{2\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta(a),\Delta(0)-\Delta(a) \}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right) 
        + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{1/2}}
    \end{align*}
    with probability $(1-\delta)$.
\end{customtheorem}



\begin{proof}
\textbf{Step 1 (Sampling rule):} First note that agnostic \sav\ 
samples by the following rule
\begin{align}
    A_\ell = \begin{cases}  \argmax_{a\in\A}\bigg\{\dfrac{\pi(a)\overline{\wsigma}_\ell(a)}{T_{\ell}(a)}\bigg\}, &\text{ if } \wZ_{\ell} \geq 0, \ell > \sqrt{n}\\
    %%%%%%%%%%%%%
    \sim \pi_e, &\text{ if } \wZ_{\ell} \geq 0, \ell \leq \sqrt{n} \\
    %%%%%%%%%%%%%
    0 &\text{ if } \wZ_{\ell} < 0 
    \end{cases} \label{eq:bandit-saver-sampling-rule-1}.
\end{align}
where, $\wZ_\ell = \sum_{\ell'=1}^{\ell-1}\wmu^c_{\ell'}\left((A_{\ell'}) - C_{\ell'}(A_{\ell'})\right) + \wmu^c_{\ell}(J_\ell) - C_\ell(J_\ell) - (1-\alpha)\ell\mu^c(0)$ is the safety budget and $J_\ell = \argmax_{a\in\A}\frac{\pi(a)\overline{\wsigma}_\ell(a)}{T_{\ell}(a)}$. Again observe that the exploration policy $\pi_e$ is a uniform sampling procedure (see \Cref{rem:pi-e}), that results in the good cost estimate of actions as defined in \eqref{eq:good-cost-event}. This is proved in \Cref{corollary:safe-conc}.


\textbf{Step 2 (MSE Decomposition):} First recall that the agnostic algorithm does not know the variances and the means. We define the good cost event when the oracle has a good estimate of the cost mean. This is stated as follows:
\begin{align*}
    \xi_{c,n} = \bigcap_{\substack{1\leq \ell \leq n,\\ 1 \leq a \leq A}}\left\{\left|\wmu^c_\ell(a)-\mu^c(a)\right|\leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_\ell(a)}}\right\}
\end{align*}
We define the good variance event as 
\begin{align}
    \xi_{v,n} = \bigcap_{\substack{1\leq \ell \leq n,\\ 1 \leq a \leq A}}\left\{|\wsigma^{}_\ell(a) - \sigma(a)|\leq (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_\ell(a)}}\right\}. \label{eq:bandit-good variance-event}
\end{align}
We define the safety budget event
\begin{align*}
    \xi_{Z,n} = \bigcap_{1\leq \ell \leq n}\left\{\wZ_{\ell} \geq 0\right\}
\end{align*}
Using the definition of MSE and \Cref{lemma:wald-variance} we can show that the MSE of \sav\ is bounded by
\begin{align*}
\L_n(\pi) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{Z,n}}\cap\indic{\xi_{c,n}}\cap\indic{\xi_{v,n}}\right]}_{\textbf{Part A, $\wZ_n \geq 0$}}%\\
%%%%%%%%%%%%%
+ \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{Z,n}}^C\right]}_{\textbf{Part B, $\wZ_n < 0$}} \\
%%%%%%%%%%%%%%%%%%%%%%
&\quad + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{c,n}}^C\right]}_{\textbf{Part C, Safety event does not hold}} + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{v,n}}^C\right]}_{\textbf{Part D, Variance event does not hold}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(a)}{\leq} \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\cap\xi_{v,n}\}\right]}{\underline{T}^2_{n}(a)} + \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi^C_{Z,n}\}\right]}{\underline{T}^2_{n}(a)} + \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi^C_{c,n}\}\right]}{\underline{T}^2_{n}(a)}\\
%%%%%%%%%%%%%%%%%%%%%
&\quad + \sum_{a=0}^A  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi^C_{v,n}\}\right]}{\underline{T}^2_{n}(a)}
\end{align*}
where, $(a)$ follows from \Cref{lemma:wald-variance}. 
Divide the total budget $n$ into two parts, $n_{f}$ when $\sum_{\ell=1}^n\indic{\wZ_\ell \geq 0}$ is true, then any action from $\{0\}\bigcup\A$ can be sampled. Hence,
$\sum_{a=0}^A\E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\cap\xi_{v,n}\}\right]=n_{f}$. 
The other part consist of $n_{u} = n-n_{f}$ samples when $\sum_{\ell=1}^n\indic{\wZ_\ell < 0}$ and only action $\{0\}$ is sampled. Hence,
$\E\left[T_{n}(0)\mathbb{I}\{\xi_{v,n}\cap\xi_{c,n}\cap\xi^C_{Z,n}\}\right]=n_{f}$. 

\textbf{Step 3 (Sampling of oracle for $\wZ_\ell \geq 0$):} First note that when $\wZ_\ell\geq 0$ the oracle samples at round $\ell$ the action $\argmax_a U_{\ell+1}(a)$ where
\begin{align}
U_{\ell+1}(a') &=\frac{\pi(a')}{T_{\ell}(a')}\overline{\wsigma}_\ell(a') \leq   \frac{\pi(a')}{T_{\ell}(a')}\left(\sigma(a') + (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(a)}}\right)\label{eq:saver-1}
%%%%%%%%%%%%%%%
\end{align}
Let $\ell+1>2 A$ be the time at which a given arm $k$ is pulled for the last time, i.e., $T_{\ell}(k)=T_{n}(k)-1$ and $T_{\ell+1}(p')=T_{n}(p')$. Note that as $n \geq 4 K$, there is at least one arm $p'$ such that this happens, i.e. such that it is pulled after the initialization phase. Since the oracle chooses to pull arm $p'$ at time $\ell+1$, we have for any arm $p$
\begin{align}
U_{\ell+1}(p) \leq U_{\ell+1}(p') .\label{eq:saver-2}
\end{align}
From \eqref{eq:oracle-1} and using the fact that $T_{\ell}(p')=T_{n}(p')-1$, we can show that
\begin{align}
U_{\ell+1}(p') \leq \frac{\pi(p')}{T_{\ell}(p')}\left(\sigma(p')+(2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_t(p')}}\right)=\frac{\pi(p')}{T_{n}(p')-1}\left(\sigma(p') + (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_n(p')-1}} \right) \label{eq:saver-3}
\end{align}
Also note that
\begin{align}
    U_{\ell+1}(p) = \frac{\pi(p)}{T_{\ell}(p)}\left(\sigma_t(p)+ (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_n(p')-1}}\right) \overset{(a)}{\geq} \frac{\pi(p)}{T_{n}(p)}\sigma(p). \label{eq:saver-4}
\end{align}
where, $(a)$ follows as $T_{\ell}(p)\leq T_{n}(p)$. 
Combining \eqref{eq:saver-2}, \eqref{eq:saver-3}, \eqref{eq:saver-4} we can show that
\begin{align}
    \frac{\pi(p)}{T_{n}(p)}\sigma(p) \leq \frac{\pi(p')}{T_{n}(p')-1}\left(\sigma(p') + (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{2 T_n(p')-1}}\right)  \label{eq:saver-5}
\end{align}
Note that in the above equation, there is no dependency on $\ell$, and thus, the probability that \eqref{eq:saver-5} holds for any $p$ and for any $p'$ such that arm $p'$ is pulled after the initialization phase, i.e., such that $T_{n}(p')>2$ depends on the probability of event $\xi_{Z,n}$.

\textbf{Step 4. (Lower bound on $T_{n}(p)$ for $\wZ_\ell \geq 0$):} 
Following step $4$ of \Cref{thm:bandit-oracle-loss} and 
using the definition of the optimal allocation $T_{n}(p')^*=n_f \frac{\pi(p') \sigma(p')}{M}$, and the fact that $T_{n}(p') \geq \bb^*(p')(n_f-2 A)+2$, \eqref{eq:saver-5} may be written as for any arm $p$
\begin{align}
\frac{\pi(p) \sigma(p)}{T_{n}(p)} & \leq \frac{\pi(p')}{T_{n}(p')^*} \frac{n_f}{(n_f-2 A)}\left(\sigma(p') + (2\eta + 4\eta^2) \sqrt{\frac{\log (A n(n+1) / \delta)}{\bb^*(p')(n_f-2 A)}} \right)\nonumber\\
%%%%%%%%%%%%%%%%%
&\leq \dfrac{M}{n_f} + \dfrac{4 A M}{n_f^2} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}}  \label{eq:saver-6}
\end{align}
because $n_f \geq 4 A$. Defining $\bb^*_{\min} = \min_a \bb^*(a)$ we can show that
\begin{align}
    \frac{\pi(p) \sigma(p)}{T_{n}(p)} \leq \dfrac{M}{n_f} + \dfrac{4 A M}{n_f^2} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} \label{eq:saver-6-0}
\end{align}
By rearranging \eqref{eq:saver-6}, we obtain the lower bound on $T_{n}(p)$ :
\begin{align}
T_{n}(p) &\geq \frac{\pi(p) \sigma(p)}{\frac{M}{n_f}+\frac{4 A M}{n_f^2} + \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}}} = \dfrac{\pi(p) \sigma(p)}{\frac{M}{n_f}\left(1 + \frac{4A}{n_f} + \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)} \nonumber\\
%%%%%%%%%%%%%%%%
&\overset{(a)}{\geq} T^*_{n}(p) - \frac{(2\eta + 4\eta^2)\bb^*(p)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}-4 A \bb(p), \label{eq:saver-6-1}
\end{align}
where in $(a)$ we use $1 /(1+x) \geq 1-x$ (for $x>-1$ ). Note that the lower bound holds on $\xi_{c,n}\cap\xi_{v,n}$ for any arm $p$.


\textbf{Step 5. (Upper bound on $T_{n}(p)$ for $\wZ_\ell \geq 0$):} Now using \eqref{eq:oracle-6-1} and the fact that $\sum_a T_{n}(a)=n_f$, we obtain
\begin{align*}
T_{n}(p)=n_f-\sum_{p' \neq p} T_{n}(p') \leq\left(n_f-\sum_{p' \neq p} T_{n}^*(p')\right)+\sum_{p' \neq p}\left(\frac{(2\eta + 4\eta^2)\bb^*(p')\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}} + 4 A \bb(p')\right) .
\end{align*}
Now since $\sum_{p' \neq p} \bb(p') \leq 1$ we can show that
\begin{align}
T_{n}(p) \leq T_{n}^*(p) + \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}} +4 A . \label{eq:saver-6-2}
\end{align}



\textbf{Step 6 (Bound part A):} We now bound the part A using \eqref{eq:saver-6}
\begin{align*}
    \sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right] &\leq
    %%%%
    \sum_{a\in\A}  \frac{\pi(a)^2\sigma(a)^2 \E\left[T_{n}(a)\mathbb{I}\{\xi_{c,n}\cap\xi_{Z,n}\}\right]}{\underline{T}^2_{n}(a)}\\
    %%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq} \left(\frac{M }{n_f}+\frac{4 A M}{n_f^2} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}}\right)^2 n_{f} \\
    %%%%%%%%%%%%%
    &\overset{}{\leq} \frac{M^2}{n_f}+\frac{8A M^2}{n_f^2} + \frac{16A^2 M^2}{n_f^3} + 2M \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} \\ 
    %%%%%%%%%%%%%%%%
    &\qquad + 8AM\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} + \dfrac{(2\eta + 4\eta^2)^2\log (A n(n+1) / \delta)}{\bb^{*,3}_{\min}n_f^{2}}
\end{align*}
where, in $(a)$ we have that $M = \sum_a \pi(a)\sigma(a)$ and $\E\left[T_{n}(a)\mathbb{I}\{\xi_{v,n}\cap\xi_{c,n}\cap\xi_{Z,n}\}\right]=n_{f}$ 
% $(b)$ follows as $n_{safe}\leq n$.


\textbf{Step 7 (Upper Bound to Constraint Violation):} In this step we bound the quantity $\C_n = \sum_{\ell=1}^n\indic{\wZ_\ell < 0, A_t\sim\{\wb_t, \pi_0\}}$. Observe that $\C_n = \sum_{\ell=1}^n\indic{\wZ_\ell < 0, A_t\sim\{\wb_t, \pi_0\}} = T_n(0)\indic{\xi^C_{Z,n}}$ as when the constraint are violated action $\{0\}$ is sampled. 
% Note that for the agnostic algorithm the constraint violation only depends on the safe events $\xi_{c,n}$. Following the same way as step 7 in \Cref{thm:bandit-oracle-loss} we can show that
\begin{align}
&n_u =T_{\tau-1}(0) = \dfrac{1}{\alpha\mu^c(0)}\left(\sum_{a=1}^A N(a)\right)\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq 
% \frac{2 A+2}{\alpha \mu^c(0)}+
\frac{2}{\alpha \mu^c(0)} \sum_{a\in\uA}
\Delta^c(a)
\left(\dfrac{\pi(a)\sigma(a)}{M}n_f \right) 
%%%%%%
+ \frac{4}{\alpha \mu^c(0)}\!\!\!\sum_{a\in\sA\setminus\{0\}}\!\!\!\left(\Delta^c(0)-\Delta^c(a) \right)\left(\dfrac{\pi(a)}{M}\left(\sigma(a) + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}}\right)n_f \right)\nonumber\\
%%%%%%%%%%%%%%%%%%
&= 
% \frac{2 A+2}{\alpha \mu^c(0)}+
\frac{6}{\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{\Delta^c(a),\Delta^c(0)-\Delta^c(a) \}\left(\dfrac{\pi(a)}{M}(n - n_u)\left(\sigma(a) + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{1/2}}\right) \right)\nonumber\\
%%%%%%%%%%%%%%%%%%
&\overset{(a)}{\leq} \dfrac{H_*}{2}\dfrac{n}{M} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{1/2}} \leq \dfrac{H_*}{2}\dfrac{n}{M} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}(n - n_u)^{1/2}} \nonumber\\
%%%%%%%%%%%%%%%%%%%%
&\leq \dfrac{H_*}{2}\dfrac{n}{M} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{1/2}}
% \nonumber\\
%%%%%%%%%%%%%%%%%%
% &= \frac{2 A+2}{\alpha \mu^c(0)H_*} + 
\label{eq:saver-11}
\end{align}
where, $(a)$ follows for $6H^2_* + 11H_* > 0$ which is satisfied for all $H_* > 0$. 
% \begin{align}
%     T_{n}(0) \leq \frac{2 A+2}{\alpha \mu^c(0)}+\frac{2\log(2/\delta)}{\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\dfrac{\pi(a)}{M}\left(\sigma(a) + \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n^{3/2}}\right)n \right)\label{eq:saver-11}
% \end{align}


% In this step we prove upper and lower bounds for  $\{0\}$ and $\wZ_\ell < 0$. Let $\tau=\max \left\{\ell \leq n \mid I_t=0\right\}$ be the last round in which the default action is played. Since $\xi_s$ holds and
% \begin{align*}
%     \wmu_t(0) + C_t(0) < \mu^*(a) < \max_a\wmu_t(a) + C_t(a).
% \end{align*}
% Note that we can sample the default action $0$ for two reasons. If the safety budget $\wZ_\ell \geq 0$ and
% $$
% \dfrac{\pi(0)\sigma(0)}{T_t(0)} > \dfrac{\pi(a)\sigma(a)}{T_t(a)}
% $$ 
% for all $a\in\A\setminus\{0\}$.  
% This is handled in steps 3 and 4. Now in this step we focus when $\wZ_\ell < 0$. Note that in this case we only sample action $0$ if $\wZ_\ell(0) < 0$. Let $J_t = \argmax_a\frac{\pi(a)\sigma(a) }{T_t(a)}$. Define the LCB for an action $a$ as $G_t(a) = \wmu_t(a) - C_t(a)$. It follows then
% \begin{align}
% \sum_{a=0}^A T_{\tau-1}(a) G_{\tau}(a)+G_{\tau}(J_\tau)-(1-\alpha) \mu(0) \tau<0 \label{eq:oracle-7}
% \end{align}
% By dropping $G_{\tau}(J_\tau)$, replacing $\tau$ with $\sum_{a=0}^A T_{\tau-1}(a)+1$, and rearranging the terms in \Cref{eq:oracle-7}, we get
% \begin{align}
% \alpha T_{\tau-1}(0) \mu(0) &<(1-\alpha) \mu(0)+\sum_{a=1}^A T_{\tau-1}(a)\left((1-\alpha) \mu(0)-G_{\tau}(a)\right) \nonumber\\
% %%%%%%%%%%%%
% & \leq(1-\alpha) \mu(0) 
% +\sum_{a=1}^A T_{\tau-1}(a)\left((1-\alpha) \mu(0)-\mu(a)+\sqrt{\frac{\log(2/\delta)}{T_{\tau-1}(a)}}\right) \nonumber\\
% %%%%%%%%%%%%
% & \leq 1+\sum_{a=1}^A N(a) \implies T_{\tau-1}(0) \leq \dfrac{1}{\alpha\mu(0)}\left(1+\sum_{a=1}^A N(a)\right) . \label{eq:oracle-8}
% \end{align}
% where $\Delta^{\alpha}(a)=(1-\alpha) \mu(0)-\mu(a)$ and
% \begin{align*}
% N(a) &=T_{\tau-1}(a) \cdot\left((1-\alpha) \mu(0)-\mu(a)+\sqrt{\log(2/\delta) / T_{\tau-1}(a)}\right) \\
% &=\Delta^{\alpha}(a) T_{\tau-1}(a)+\sqrt{\log(2/\delta) T_{\tau-1}(a)}
% \end{align*}
% is a bound on the decrease in $\wZ_\tau$ in the first $\tau-1$ rounds due to choosing action $a$. We will now bound $N(a)$ for each $a>0$. Now observe
% \begin{align*}
%     \Delta^{\alpha}(a) = (1-\alpha) \mu(0)-\mu(a) = \mu(0) - \alpha\mu(0) - \mu(a) = -(\mu^* - \mu(0)) - \alpha\mu(0) + (\mu^* - \mu(a)) = -\Delta(0) - \alpha\mu(0) + \Delta(a).
% \end{align*}
% where, $\mu^* = \max_a\mu(a)$. The first case is $\Delta^{\alpha}(a) > 0$, i.e. $\Delta(a) > \Delta(0)+\alpha \mu(0)$. These are the unsafe actions (see the definition of $\Delta^\alpha(a))$ we have from \eqref{eq:oracle-6-2}
% \begin{align*}
%     T_n(a) &\leq T^*_n(a) + 8A
%     %%%%%%%%%%%%
%     = \dfrac{\pi(a)\sigma(a)}{M}n +  8A
% \end{align*}
% Plugging this back in $N(a)$ we get
% \begin{align}
%     N(a) &=\Delta^{\alpha}(a) T_{\tau-1}(a)+\sqrt{\log(2/\delta) T_{\tau-1}(a)} \nonumber\\
%     %%%%%%%%%%%%%%%%%%%
%     &\leq \dfrac{\pi(a)\sigma(a)}{M}n\Delta^{\alpha}(a) + 8A\Delta^{\alpha}(a) + \sqrt{\log(2/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n + 8A\right)} \nonumber\\
%     %%%%%%%%%%%%%%%%%%%%%
%     &\overset{(a)}{\leq} \dfrac{1}{\Delta^{\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n + 8A\right) + \sqrt{\log(2/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n + 8A\right)} \label{eq:oracle-9} 
% \end{align}
% where, $(a)$ follows as $\Delta^{\alpha}(a) > 0$.
% The other case is $\Delta^{\alpha}(a)< 0$, i.e. $\Delta(a)<\Delta(0)+\alpha \mu(0)$ then only safe actions are pulled. Then
% \begin{align}
% N(a) &\leq -\Delta^{\alpha}(a)T_{\tau-1}(a) + \sqrt{\log(2/\delta) T_{\tau-1}(a)} = \underbrace{-\Delta^{\alpha}(a)}_{a}T_{\tau-1}(a) + \underbrace{\sqrt{\log(2/\delta)}}_{b}\sqrt{T_{\tau-1}(a)}\nonumber\\
% %%%%%%%%%%%%%%%%%%
% &\overset{(a)}{\leq} -\dfrac{\log(2/\delta)}{4\Delta^{\alpha}(a)} = \dfrac{\log(2/\delta)}{4(\Delta(0) + \alpha\mu(0) - \Delta(a))}%\\
% %%%%%%%%%%%%%%%%%%%
% \label{eq:oracle-10}
% \end{align}
% where, $(a)$ follows by using $a x^2+b x \leq-b^2 / 4 a$ for $a<0$. 
% Summarizing \eqref{eq:oracle-9} to \eqref{eq:oracle-10} for $a\in\uA$ gives
% \begin{align*}
% N(a) &\leq \dfrac{1}{\Delta^{\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n + 8A\right) + \sqrt{\log(2/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n + 8A\right)}\\
% %%%%%%%%%%%%%%%%%%
% &\overset{(a)}{\leq} \dfrac{1}{\Delta^{\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n\right) + \sqrt{\log(2/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)}\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &\overset{(b)}{\leq} \dfrac{1}{\Delta^{\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M }n \right) + \log(2/\delta)\left(\dfrac{\pi(a)\sigma(a)}{M }n \right)\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &\overset{(c)}{\leq} \dfrac{2\log(2/\delta)}{\Delta^{\alpha}(a)}\left(\dfrac{\pi(a)\sigma(a)}{M }n\right) 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% \end{align*}
% where, $(a)$ follows as $A\leq \sqrt{n}$ so we can subsume the $8A$ into the leading term $\sqrt{n\log(2/\delta)}$, 
% $(b)$ follows as 
% \begin{align*}
%     \left(\dfrac{\pi(a)\sigma(a)}{M }n\right) \geq \sqrt{\left(\dfrac{\pi(a)\sigma(a)}{M }n \right)}.
% \end{align*}
% The $(c)$ follows as $\max\{\log(2/\delta),\Delta^\alpha(a)\}\leq 2\log(2/\delta)/\Delta^\alpha(a)$. Similarly for $a\in\sA$ we can show that
% \begin{align*}
%     N(a) \leq \dfrac{\log(2/\delta)}{4(\Delta(0) + \alpha\mu(0) - \Delta(a))} \overset{(a)}{\leq} \dfrac{2\log(2/\delta)}{4(\Delta(0) + \alpha\mu(0) - \Delta(a))}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)
% \end{align*}
% where, $(a)$ follows by inserting $\left(\frac{\pi(a)\sigma(a)}{M}n \right) >1$ for the quantity $\frac{2\log(2/\delta)}{4(\Delta(0) + \alpha\mu(0) - \Delta(a))}$. Observe that this term consists of the safe action, so we insert $\left(\frac{\pi(a)\sigma(a)}{M}n\right)$. Plugging everything back in \eqref{eq:oracle-10}, we get
% \begin{align}
% T_{n}(0) =T_{\tau-1}(0)+1 &= \dfrac{1}{\alpha\mu(0)}\left(1+\sum_{a=1}^A N(a)\right)\nonumber\\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% &\leq \frac{2 A+2}{\alpha \mu(0)}+\frac{1}{\alpha \mu(0)} \sum_{a\in\uA}\dfrac{2\log(2/\delta)}{\Delta(a)}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right) 
% %%%%%%
% + \frac{1}{\alpha \mu(0)}\sum_{a\in\sA\setminus\{0\}}\dfrac{2\log(2/\delta)}{\Delta(0)-\Delta(a) }\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)\nonumber\\
% &= \frac{2 A+2}{\alpha \mu(0)}+\frac{2\log(2/\delta)}{\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)\label{eq:oracle-11}
% \end{align}
% Observe, that for safe action small $\Delta(0) - \Delta(a)$ implies that action $a$ is close to the $\mu(0)$. This implies that safe action close to the $\mu(0)$ is allocated more samples.

\textbf{Step 8 (Lower bound to Constraint violation):} To bound the lower bound of $T_n(0)$ for $\wZ_\ell < 0$ we equate the safety budget to $0$. Define $\underline{G}(n_f,a) \coloneqq \frac{(2\eta + 4\eta^2)\bb^*(a)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}$.
%
Observe that from \eqref{eq:saver-6-1} and \eqref{eq:saver-11} we get
\begin{align}
&T_{\tau-1}(0) \geq  \dfrac{1}{\alpha\mu^c(0)}\left(1 + \sum_{a=1}^A N(a)\right) %\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\overset{(a)}{\geq} 1 +  \frac{1}{\alpha \mu^c(0)} \sum_{a\in\uA}\Delta^c(a)\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - \underline{G}(n_f,a) - 4A\bb^*(a)\right) \nonumber\\
%%%%%
&\quad +
\frac{1}{\alpha \mu^c(0)}\sum_{a\in\sA\setminus\{0\}}(\Delta^c(0)-\Delta^c(a) )\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - \underline{G}(n_f,a) - 4A\bb^*(a)\right) 
\nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%
&\geq 1 + \frac{1}{8\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\left(\dfrac{\pi(a)\sigma(a)}{M}n_f - \underline{G}(n_f, a) - 4A\bb^*(a)\right) \nonumber\\
%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(b)}{=} \dfrac{H_*}{8}\dfrac{n_f}{M} - \frac{A}{2\alpha \mu^c(0)} \sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\bb^*(a) - \underline{G}(n_f,a)
\nonumber\\
%%%%%%%%%%%%%%%%%%%%
&\overset{(c)}{=} \dfrac{n_f}{M}\left(\dfrac{H_*}{8} - \dfrac{M}{n_f}\left(\frac{A}{2\alpha \mu^c(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\bb^*(a) - \underline{G}(n_f,a)\right) \right) \label{eq:saver-11-1}
\end{align}
where, $(a)$ follows as $\alpha \mu^c(0) \geq 1$, $(b)$ follows from the definition of $H_*$. Observe that from
\eqref{eq:saver-11-1} we have that

\begin{align*}
    T_n(0) &\overset{(a)}{\geq} \dfrac{n_f}{M}\bigg(\dfrac{H_*}{8}  - \dfrac{M}{n_f}\bigg(\frac{A}{2\alpha \mu^c(0)}\sum_{a\in\A\setminus\{0\}}\min^{+}\{(\Delta^c(a),\Delta^c(0)-\Delta^c(a)) \}\dfrac{\pi(a)\sigma(a) n_f}{M} \\
    %%%%
    &\quad - \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\dfrac{\pi(a)\sigma(a)}{M}n_f\bigg) \bigg)%\\
    %%%%%%%%%%%%%%%
    = \dfrac{n_f}{M}\left(\dfrac{H_*}{8} - \frac{A}{2}\dfrac{H_*}{M} - \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}  \right).
    % \overset{(a)}{\geq} \left(1 - \dfrac{A}{4M} + \dfrac{H_*}{8}\right)\dfrac{n_f}{M}
\end{align*}
where, $(a)$ follows for $\bb^*(a) = \frac{\pi(a)\sigma(a)}{M}n_f$.



% we have (following step 6 of the previous theorem) that
% \begin{align*}
%     % T_n(0) &\geq \min\left\{T^*_{n}(0)-4 A \bb(0), \frac{2 A+2}{\alpha \mu(0)}+\frac{2\log(2/\delta)}{\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\min\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)\right\}\\
%     % %%%%%%%%%%%%%%%%%
%     % &\geq \min\left\{\dfrac{\pi(0)\sigma(0)}{M}n-4 A \bb(0), \frac{2\log(2/\delta)}{\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\min\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)\right\}\\
%     % %%%%%%%%%%%%%%%%%
%     % &\geq \dfrac{n}{M}\min\left\{\pi(0)\sigma(0)-\dfrac{4 A \bb(0)M}{n}, \frac{2\log(2/\delta)}{\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\min\{\Delta(a),\Delta(0)-\Delta(a) \}}\right\}\\
%     %%%%%%%%%%%%%%%%
%     \dfrac{T_n(0)}{\pi(0)\sigma(0)} 
%     % &\geq \dfrac{n}{M}\min\left\{1 - \dfrac{4 A \bb(0)M}{\pi(0)\sigma(0) n},\frac{2\log(2/\delta)}{\alpha \mu(0)\pi(0)\sigma(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\min\{\Delta(a),\Delta(0)-\Delta(a) \}}\right\}\\
%     %%%%%%%%%%%%%%%%%%
%     &\geq \dfrac{n}{M}\left(\frac{2\log(An(n+1)/\delta)}{\alpha \mu^c(0)\pi(0)\sigma(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\min\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\pi(a)\sigma(a) - 4A\bb(a)\dfrac{M}{n}\right)\right)
% \end{align*}
% % where, the final inequality follows for $n\geq 8A\bb(0)M/\pi(0)\sigma(0)$. 

\textbf{Step 9 (Bound Part B)}: Then from \eqref{eq:saver-11-1} we can show that
\begin{align*}
   \dfrac{\pi(0)\sigma(0)}{T_n(0)} &\leq \dfrac{M }{n_f}\dfrac{\pi(0)\sigma(0)}{  \dfrac{H_*}{8} - \dfrac{A H_*}{2M} - \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}  }\\
   %%%%%%%%%%%%%%%%%
   &\overset{}{\leq} \dfrac{M \pi(0)\sigma(0)}{n_f}\left(2 + \dfrac{H_*}{8} + \dfrac{A H_*}{2M} + \frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)\\
   %%%%%%%%%%%%%%%%
   &\overset{(a)}{\leq} \dfrac{M A \pi(0)\sigma(0)}{n_f}\left(2 + H_*\right) + \dfrac{M \pi(0)\sigma(0)}{n_f}\left(\frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)
\end{align*}
where, $(a)$ follows for $A\geq 2$.
% $1/1+m \leq 2 + m$ for $ m\geq 0$. 
It follows then by setting $\E\left[T_{n}(0)\indic{\xi^C_{Z,n}}\right]\leq n_u$ and setting $n_f = n - n_u$ that 
\begin{align*}
    &\frac{\pi(0)^2 \sigma(0)^2 \E\left[T_{n}(0)\indic{\xi_{Z,n}}^C\right]}{\underline{T}^2_{n}(0)} 
    %%%%%%%%%%%%%%%%%%%%%%
     = \dfrac{M^2 A^2 \pi^2(0)\sigma^2(0) n_u}{(n-n_u)^2}\left(2 + H_*\right)^2 + \dfrac{M^2 \pi^2(0)\sigma^2(0)}{(n - n_u)^2}\left(\frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)^2n_u\\
    %%%%%%%%%%%%%%%%%%%%%
    &\quad + 2\dfrac{M A \pi(0)\sigma(0)}{n - n_u}\left(2 + H_*\right) \cdot \dfrac{M \pi(0)\sigma(0)}{n - n_u}\left(\frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)n_u\\
    %%%%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq } \dfrac{M^2 A^2 \pi^2(0)\sigma^2(0) H_* n}{(n-H_*n)^2}\left(2 + H_*\right)^2 + \dfrac{M^2 \pi^2(0)\sigma^2(0)}{(n - H_* n)^2}\left(\frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)^2H_* n\\
    %%%%%%%%%%%%%%
    &\quad + 2\dfrac{M A \pi(0)\sigma(0)}{n - H_* n}\left(2 + H_*\right) \cdot \dfrac{M \pi(0)\sigma(0)}{n - H_* n}\left(\frac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{M\bb^{*,3/2}_{\min}n_f^{3/2}}\right)H_* n\\
    %%%%%%%%%%%%%%%%%%%%
    &\leq \dfrac{M^2 A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 5/2}_{\min}n^{5/2}}\right) + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 3/2}_{\min}n^{3/2}}\right)
\end{align*}
where, $(a)$ follows from \eqref{eq:saver-11}.












% Then we can show that
% \begin{align*}
%    \dfrac{\pi(0)\sigma(0)}{T_n(0)} &\leq \dfrac{M}{n}\dfrac{1}{ \frac{2\log(An(n+1)/\delta)}{\alpha \mu^c(0)\pi(0)\sigma(0)} \sum_{a\in\A\setminus\{0\}}\left(\frac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a)\} - 4A\bb(a)\frac{M}{n} }  - 4A\bb(a)\frac{M}{n}\right)  }\\
%    %%%%%%%%%%%%%%%%%
%    &\leq \dfrac{M}{n}\left(2 + \frac{2\log(An(n+1)/\delta)}{\alpha \mu^c(0)\pi(0)\sigma(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}\right)
% \end{align*}
% It follows then by setting $\E\left[T_{n}(0)\indic{\xi_{Z,n}^C}\right]\leq n$ that 
% \begin{align*}
%     &\frac{\pi(0)^2 \sigma(0)^2 \E\left[T_{n}(0)\indic{\cap\xi_{Z,n}^C}\right]}{\underline{T}^2_{n}(0)} 
%     \leq \dfrac{M^2}{n^2}\left(2 + \frac{2\log(An(n+1)/\delta)}{\alpha \mu^c(0)\pi(0)\sigma(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}\right)^2 n\\
%     %%%%%%%%%%%%%%%%%%%%
%     &= \dfrac{M^2}{n^2}\bigg(4 + \dfrac{8\log(An(n+1)/\delta)}{\alpha \mu^c(0)\pi(0)\sigma(0)}\sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}} \\
%     %%%
%     &\quad + \frac{4\log^2(An(n+1)/\delta)}{\alpha^2 \mu^{c,(2)}(0)\pi^2(0)\sigma^2(0)}\left(\sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}\right)^2\bigg)\\
%     %%%%%%%%%%%%%%%%%%%%%%
%     &\overset{(a)}{=} \dfrac{M^2}{n^2}\left(4 + \dfrac{8\log(An(n+1)/\delta) H_*}{\pi(0)\sigma(0)} + \frac{4H^2_*\log(An(n+1)/\delta)}{\pi^2(0)\sigma^2(0)}\right)
% %     &\overset{(a)}{\leq}\frac{\pi(0)^2 \sigma(0)^2 \E\left[T_{n}(0)\indic{\xi_{s,n}}\right]}{\underline{T}^2_{n}(0)}\underbrace{\E\left[\indic{\xi_{Z,n}}^C\right]}_{\textbf{Total Safety violation}}\\
% %     %%%%%%%%%%%%%%%%%%%%
% %     &\leq \frac{2 A+2}{\alpha \mu(0)}+\frac{2\log(2/\delta)}{\alpha \mu(0)} \sum_{a\in\A\setminus\{0\}}\dfrac{1}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}\left(\dfrac{\pi(a)\sigma(a)}{M}n \right)
% \end{align*}
% where, in $(a)$ the $H_*$ is a problem dependent parameter defined as 
% \begin{align*}
%     H_* = \frac{1}{\alpha\mu(0)}\sum_{a\in\A\setminus\{0\}}\dfrac{\pi(a)\sigma(a)}{\max\{\Delta(a),\Delta(0)-\Delta(a) \}}
% \end{align*}


\textbf{Step 10 (Combine everything):} Combining everything from step 5, step 8 and setting $\delta=1/n^2$ we can show that the MSE of oracle scales as
\begin{align}
    \L_n(\pi) &\leq \frac{M^2}{n_f}+\frac{8A M^2}{n_f^2} + \frac{16A^2 M^2}{n_f^3} + 2M \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} \nonumber\\ 
    %%%%%%%%%
    &\qquad + 8AM\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} + \dfrac{(2\eta + 4\eta^2)^2\log (A n(n+1) / \delta)}{\bb^{*,3}(p')n_f^{2}}\nonumber\\
    %%%%%%%%%%
    &\qquad + \dfrac{M^2 A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 5/2}_{\min}n^{5/2}}\right) + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 3/2}_{\min}n^{3/2}}\right)\nonumber\\
    %%%%%%%%%%%%%%%%%%%
    &\qquad 
    % + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{Z,n}}^C\right]}_{\textbf{Part B, $\wZ_n < 0$}} 
    + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{c,n}}^C\right]}_{\textbf{Part C, Safety event does not hold}}%\\
    + \underbrace{\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu_{n}(a)-\mu(a)\right)^2\indic{\xi_{v,n}}^C\right]}_{\textbf{Part D, Variance event does not hold}}\nonumber%\\
\end{align}
\begin{align}
    %%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%
    &\overset{(a)}{\leq} \frac{M^2}{n_f}+\frac{8A M^2}{n_f^2} + \frac{16A^2 M^2}{n_f^3} + 2M \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} \nonumber\\ 
    %%%%%%%%%
    &\qquad + 8AM\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n_f^{3/2}} + \dfrac{(2\eta + 4\eta^2)^2\log (A n(n+1) / \delta)}{\bb^{*,3}_{\min} n_f^{2}}\nonumber\\
    %%%%%%%%%%
    &\qquad + \dfrac{M^2 A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 5/2}_{\min}n^{5/2}}\right) + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 3/2}_{\min}n^{3/2}}\right)
    %%%%%%%%%%%%%%%%
    + 3\sum_{\ell=1}^n\dfrac{2\eta + 4\eta^2}{n^2}\nonumber\\
    %%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%
    &\overset{(b)}{\leq} \frac{M^2}{n}+\frac{8A M^2}{n^2} + \frac{16A^2 M^3}{n^3} + 2M^{5/2} \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{3/2}} \nonumber\\ 
    %%%%%%%%%
    &\qquad + 8AM^{5/2}\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{3/2}} + \dfrac{M^2(2\eta + 4\eta^2)^2\log (A n(n+1) / \delta)}{\bb^{*,3}_{\min} n^2}\nonumber\\
    %%%%%%%%%%
    &\qquad + \dfrac{M^2 A^2\pi^2(0)\sigma^2(0)}{n}\left(2 + H_*\right)^2 + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 5/2}_{\min}n^{5/2}}\right) + O\left(\dfrac{\sqrt{H_*^2\log (A n(n+1) / \delta)}}{\bb^{*, 3/2}_{\min}n^{3/2}}\right)
    %%%%%%%%%%%%%%%%
    + \dfrac{2}{n}\label{eq:bandit-final-loss-saver}
\end{align}
where, $(a)$ follows as $\sum_{a=0}^A \pi(a)^2 \E_{\D}\left[\left(\wmu^c_{n}(a)-\mu^c(a)\right)^2\right] \leq 2\eta + 4\eta^2$ and using the low error probability of the cost event from \Cref{lemma:conc-mu} and variance event from \Cref{corollary:conc-var}. The $(b)$ follows by substituting $n_u \leq \frac{H_*}{2}\frac{n}{M}$ and considering the leading terms. 
The claim of the theorem follows.
\end{proof}


\subsection{Bandit Regret Corollary}
\label{app:bandit-regret-corollary}


\begin{customcorollary}{1}\textbf{(formal)}
The constraint regret is given by $\cR^c_n \leq O\left(\frac{\log(n)}{\bb^{*,3/2}_{\min}n^{1/2}}\right)$ and the reward regret is given by $\cR_n \leq O\left(\frac{\log(n)}{\bb^{*,3/2}_{\min}n^{3/2}}\right)$.

% \begin{align*}
%     \cR_n \leq O\left(\frac{\log(n)}{\bb^{*,3/2}_{\min}n^{1/2}}\right)
% \end{align*}
\end{customcorollary}


\begin{proof}
    The upper bound to the oracle constraint is given by \eqref{eq:bandit-constraint-lower-bound} as follows
    \begin{align*}
        \C_n(\pi) \leq \dfrac{H_*}{2}\dfrac{n}{M}
        % \geq \dfrac{n_f}{M}\left(\dfrac{H_*}{8} - \frac{A}{2}\dfrac{H_*}{M}  \right) 
    \end{align*}
    The upper bound to the constraint violation of \sav\ is given by \eqref{eq:saver-11}
    \begin{align*}
        \C_n(\pi) \leq \dfrac{H_*}{2}\dfrac{n}{M} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{1/2}} 
        % = \dfrac{H_*}{2}\dfrac{n}{M} + \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}_{\min}n^{3/2}(2M - H_*)^{3/2}}
    \end{align*}
    Hence, from the constraint regret definition, we can show that
    \begin{align*}
        \cR^c_n = \C_n(\pi) - \overline{\C}^*_n(\pi) \leq O\left(\frac{\log n}{\bb^{*,3/2}_{\min}n^{1/2}}\right)
    \end{align*}
% \end{proof}




% \begin{customcorollary}{2}
% The reward regret is given by
% \begin{align*}
%     \R_n \leq O\left(\dfrac{\log(n)}{\bb^{*,3/2}_{\min}n^{3/2}}\right)
% \end{align*}
% \end{customcorollary}


% \begin{proof}
    Observe that the MSE of the agnostic algorithm \sav\ is given by \eqref{eq:bandit-final-loss-saver} and the upper bound to the oracle MSE is given by \eqref{eq:bandit-final-loss-oracle}. Comparing these two MSE directly leads to the reward regret as follows:
    \begin{align*}
    \cR_n = \L_n(\pi) - \overline{\L}^*_n(\pi) = 
%     \L_n(\pi) &\leq  \frac{M^2}{n}+\frac{16A M^2}{n^2} + \frac{16A^2 M^2}{n^3} + 2M \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}(k)n^{3/2}} \\ 
%     %%%%%%%%%%%%%%%%
%     &\qquad + 8AM\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n(n+1) / \delta)}}{\bb^{*,3/2}(k)n^{3/2}} + \dfrac{(2\eta + 4\eta^2)^2\log (A n(n+1) / \delta)}{\bb^{3}(k)n^{2}} \\
%     %%%%%%%%%%%%%%%%%%
%     &\qquad + \dfrac{M^2}{n}\left(4 + \dfrac{8\log(2/\delta) H_*}{\alpha \mu(0)\pi(0)\sigma(0)} + \frac{4H^2_*\log(2/\delta)}{\alpha^2 \mu^2(0)\pi^2(0)\sigma^2(0)}\right)
%     %%%%%%%%%%%%%%%%
%     + 3\sum_{\ell=1}^n\dfrac{2\eta + 4\eta^2}{n^2}%\\
% \end{align*}
% \begin{align*}
%     %%%%%%%%%%%%%%%%%%%%%%%
%     %%%%%%%%%%%%%%%%%%%%%%%%
%     \L_n(\pi) - &\left(\frac{M^2}{n}+\frac{16A M^2}{n^2} + \frac{16A^2 M^2}{n^3} + \dfrac{M^2}{n}\left(4 + \dfrac{16\log(2n) H_*}{\alpha \mu(0)\pi(0)\sigma(0)} + \frac{8H^2_*\log(2n)}{\alpha^2 \mu^2(0)\pi^2(0)\sigma^2(0)}\right) + \dfrac{2\eta + 4\eta^2}{n}\right)\\
%     %%%%%%%%%%%%%%
%     &\leq 2M \dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n^2(n+1))}}{\bb^{*,3/2}(k)n^{3/2}} + \dfrac{8AM}{n}\dfrac{(2\eta + 4\eta^2)\sqrt{\log (A n^2(n+1) )}}{\bb^{*,3/2}(k)n^{3/2}} + \dfrac{(2\eta + 4\eta^2)^2\log (A n^2(n+1))}{\bb^{3}(k)n^{2}}\\
%     %%%%%%%%%%%%%%%%
%     &\qquad + \dfrac{2\eta + 4\eta^2}{n^2}
%     \end{align*}
%     by choosing $\delta = 1/n^2$
% Hence, it follows that
% \begin{align*}
O\left(\dfrac{\log(n)}{\bb^{*,3/2}_{\min}n^{3/2}}\right)
\end{align*}
\end{proof}





==> tree_mdp_loss.tex <==
In this section, we approximate the solution in $\T$ to DAG $\G$ and formulate the safe algorithm for policy evaluation. Recall that in a DAG $\G$ we have a cyclical dependency following \Cref{lemma:dag}. We can approximate the optimal sampling proportion that ignores the multiple path problem in $\G$ by using the tree formulation in the following way: At every time $t$ during a trajectory $\tau^k$ call the \Cref{alg:revar-g-1} to estimate $M_0(s)$ where $M_{t'}(s)\in\mathbb{R}^{L\times |\S|}$ stores the expected standard deviation of the state $s$ at iteration $t'$. 
%
After $L$ such iteration we use the value $B_0(s)$ to estimate $\bb(a|s)$ as follows:
\begin{align*}
    \bb^*(a|s) \!&\propto\! 
    \! \sqrt{\! \pi^2(a|s)\! \bigg[\sigma^2(s, a)\!  +\!    \gamma^2\!\!  \sum\limits_{s'}\!\!P(s'|s, a) M^2_0(s)\! \bigg]}.
\end{align*}
Note that for a terminal state $s$ we have the transition probability $P(s'|s, a) = 0$ and  then the $b(a|s) = \pi(a|s)\sigma(s,a)$. This iterative procedure follows from the tree formulation in \Cref{lemma:L-step-tree} and is necessary in $\G$ to take into account the multiple paths to a particular state. Also observe that in \Cref{alg:revar-g-1} we use value-iteration for the episodic setting \citep{sutton2018reinforcement} to estimate the optimal sampling proportion iteratively. The following algorithm shows the pseudocode of this iterative procedure.
%
% Hence, we do an approximation of the optimal sampling proportion in $\G$ by using the tree formulation from \Cref{thm:L-step-tree}. However, since there are multiple paths to the same state in $\G$ we have to iteratively compute the normalization factor $B$. To do this we use the following \Cref{alg:revar-g}.
%
\begin{algorithm}
\caption{Estimate $B_0(s)$ for $\G$}
\label{alg:revar-g-1}
\begin{algorithmic}[1]
\STATE Initialize $B_L(s)=0$ for all $s\in\S$ 
\FOR{$t'\in L-1, \ldots, 0$} 
\STATE $B_{t'}(s) = \sum\limits_{a} \sqrt{\pi^2(a|s)\!\left(\sigma^2(s,\! a) + \gamma^2\sum\limits_{s'}P(s'|s, a) B_{t'+1}^2(s)\right)}$
\ENDFOR
\STATE \textbf{Return} $B_0$.
\end{algorithmic}
\end{algorithm}

Finally, the safe algorithm in $\G$ can be stated as follows: At episode $k$ 
\begin{align}
\quad \text{Play } \bb^k = \begin{cases} \pi_e & \text{ if }             \wZ^k \geq 0, k \leq \sqrt{K}\\
            %%%%%%%%%%%
            \pi_{\wb^k} & \text{ if } \wZ^k \geq 0, k > \sqrt{K}\\
             %%%%%%%%%%%%
            \pi_0 &\text{ if } \wZ^k < 0 \label{eq:mdp-saver-dag-sample}
\end{cases} 
\end{align}
where $\pi_{\wb^k}$ for the episode $k$ is defined as follows: For each time $\ell=1,2,\ldots,L$ sample action $A^k_\ell = \argmax_a\tfrac{\wb^k(a|s^\ell_j)}{T^k_\ell(s^\ell_j,a)}$, where $\wb^k(a|s^\ell_j)$ is the plug-in estimate of $\bb^*(a|s^\ell_j)$ that is obtained using \Cref{alg:revar-g-1}.
